How Far Back Should a Transformer Look? Repetition and Copying in Music Sequence Models

We investigate how predictive performance depends on the maximum context available to an autoregressive model of symbolic music, and what information long-context models exploit. A small causal Transformer is trained separately at each context length T in {6, 18, 48, 96, 192, 336} and evaluated on the same target positions, both over raw tokens and over non-overlapping binary latent codes. On Nottingham folk tunes, the token predictor's test NLL decreases by 71% (0.986 bits per token) between 6 and 336 tokens, and by 71% on the O'Neill's tunes long enough for the same sweep (129 of 302 test tunes). Most of the long-context gain is explained by exact copying: the improvement appears when an earlier occurrence of the target's 16-token history enters the available context; overwriting that occurrence removes the gain, whereas equally large unrelated corruption does not; and a simple copy baseline recovers 94% of the reduction. A trained 336-token model likewise loses most of this gain when its history is restricted to recent tokens at test time. Because many repeats arise from written repeat signs expanded in the score, this result pertains specifically to these rendered score representations. By contrast, on MAESTRO performances and MusicNet scores, where exact repeats are substantially less frequent, the reduction is smaller (9% and 18%) and is largely attained by 96 tokens. Finally, an audit of an earlier draft that reported saturation at 16 tokens identified split leakage, overlapping latent receptive fields, an averaging predictor, and a per-file tempo grid; we present these as methodological checks for context-length measurements.

==> tables/numbers.tex <==
% generated by scripts/make_paper_tables.py; do not edit
\makeatletter
\newcommand{\R}[1]{\@ifundefined{R@#1}{\textbf{??#1}}{\csname R@#1\endcsname}}
\expandafter\def\csname R@aeseed/1/acc\endcsname{99.93}
\expandafter\def\csname R@aeseed/1/drop\endcsname{48}
\expandafter\def\csname R@aeseed/18/psd\endcsname{0.002}
\expandafter\def\csname R@aeseed/18/sd\endcsname{0.011}
\expandafter\def\csname R@aeseed/192/psd\endcsname{0.015}
\expandafter\def\csname R@aeseed/192/sd\endcsname{0.008}
\expandafter\def\csname R@aeseed/2/acc\endcsname{99.91}
\expandafter\def\csname R@aeseed/2/drop\endcsname{43}
\expandafter\def\csname R@aeseed/336/psd\endcsname{0.009}
\expandafter\def\csname R@aeseed/336/sd\endcsname{0.024}
\expandafter\def\csname R@aeseed/42/drop\endcsname{45}
\expandafter\def\csname R@aeseed/48/psd\endcsname{0.005}
\expandafter\def\csname R@aeseed/48/sd\endcsname{0.011}
\expandafter\def\csname R@aeseed/6/psd\endcsname{0.002}
\expandafter\def\csname R@aeseed/6/sd\endcsname{0.008}
\expandafter\def\csname R@aeseed/96/psd\endcsname{0.004}
\expandafter\def\csname R@aeseed/96/sd\endcsname{0.011}
\expandafter\def\csname R@aeseed/drop/max\endcsname{48}
\expandafter\def\csname R@aeseed/drop/min\endcsname{43}
\expandafter\def\csname R@aeseed/larger\endcsname{5}
\expandafter\def\csname R@aeseed/n\endcsname{3}
\expandafter\def\csname R@aeseed/psd/max\endcsname{0.015}
\expandafter\def\csname R@aeseed/psd/min\endcsname{0.002}
\expandafter\def\csname R@aeseed/sd/max\endcsname{0.024}
\expandafter\def\csname R@aeseed/sd/min\endcsname{0.008}
\expandafter\def\csname R@cap/done\endcsname{9}
\expandafter\def\csname R@cap/maxgain\endcsname{0.006}
\expandafter\def\csname R@cap/maxloss\endcsname{0.071}
\expandafter\def\csname R@cap/n\endcsname{9}
\expandafter\def\csname R@cap/small\endcsname{Eight}
\expandafter\def\csname R@common/maes\endcsname{0.8}
\expandafter\def\csname R@common/music\endcsname{10.4}
\expandafter\def\csname R@common/nott\endcsname{71.8}
\expandafter\def\csname R@common/oneill\endcsname{73.5}
\expandafter\def\csname R@cor/draws/n\endcsname{5}
\expandafter\def\csname R@cor/draws/t/clean/max\endcsname{0.188}
\expandafter\def\csname R@cor/draws/t/clean/min\endcsname{0.188}
\expandafter\def\csname R@cor/draws/t/control/max\endcsname{0.188}
\expandafter\def\csname R@cor/draws/t/control/min\endcsname{0.187}
\expandafter\def\csname R@cor/draws/t/erased/max\endcsname{1.060}
\expandafter\def\csname R@cor/draws/t/erased/min\endcsname{1.058}
\expandafter\def\csname R@cor/draws/t/pswap/max\endcsname{62.4}
\expandafter\def\csname R@cor/draws/t/pswap/min\endcsname{62.0}
\expandafter\def\csname R@cor/l/192/clean\endcsname{0.37}
\expandafter\def\csname R@cor/l/192/control\endcsname{0.38}
\expandafter\def\csname R@cor/l/192/erased\endcsname{0.87}
\expandafter\def\csname R@cor/l/192/n\endcsname{2783}
\expandafter\def\csname R@cor/l/192/occ\endcsname{1.3}
\expandafter\def\csname R@cor/l/336/clean\endcsname{0.35}
\expandafter\def\csname R@cor/l/336/control\endcsname{0.35}
\expandafter\def\csname R@cor/l/336/erased\endcsname{0.81}
\expandafter\def\csname R@cor/l/336/n\endcsname{3747}
\expandafter\def\csname R@cor/l/336/occ\endcsname{1.8}
\expandafter\def\csname R@cor/oneill/draws/n\endcsname{5}
\expandafter\def\csname R@cor/oneill/draws/t/clean/max\endcsname{0.223}
\expandafter\def\csname R@cor/oneill/draws/t/clean/min\endcsname{0.223}
\expandafter\def\csname R@cor/oneill/draws/t/control/max\endcsname{0.224}
\expandafter\def\csname R@cor/oneill/draws/t/control/min\endcsname{0.223}
\expandafter\def\csname R@cor/oneill/draws/t/erased/max\endcsname{1.246}
\expandafter\def\csname R@cor/oneill/draws/t/erased/min\endcsname{1.244}
\expandafter\def\csname R@cor/oneill/draws/t/pswap/max\endcsname{71.1}
\expandafter\def\csname R@cor/oneill/draws/t/pswap/min\endcsname{71.0}
\expandafter\def\csname R@cor/oneill/l/192/clean\endcsname{0.47}
\expandafter\def\csname R@cor/oneill/l/192/control\endcsname{0.47}
\expandafter\def\csname R@cor/oneill/l/192/erased\endcsname{0.78}
\expandafter\def\csname R@cor/oneill/l/192/n\endcsname{5421}
\expandafter\def\csname R@cor/oneill/l/192/occ\endcsname{1.2}
\expandafter\def\csname R@cor/oneill/l/336/clean\endcsname{0.33}
\expandafter\def\csname R@cor/oneill/l/336/control\endcsname{0.33}
\expandafter\def\csname R@cor/oneill/l/336/erased\endcsname{0.71}
\expandafter\def\csname R@cor/oneill/l/336/n\endcsname{8942}
\expandafter\def\csname R@cor/oneill/l/336/occ\endcsname{1.9}
\expandafter\def\csname R@cor/oneill/t/192/clean\endcsname{0.37}
\expandafter\def\csname R@cor/oneill/t/192/control\endcsname{0.38}
\expandafter\def\csname R@cor/oneill/t/192/erased\endcsname{1.28}
\expandafter\def\csname R@cor/oneill/t/192/n\endcsname{31068}
\expandafter\def\csname R@cor/oneill/t/192/occ\endcsname{1.2}
\expandafter\def\csname R@cor/oneill/t/192/pnew/clean\endcsname{0.8}
\expandafter\def\csname R@cor/oneill/t/192/pnew/swap\endcsname{51}
\expandafter\def\csname R@cor/oneill/t/336/clean\endcsname{0.22}
\expandafter\def\csname R@cor/oneill/t/336/control\endcsname{0.22}
\expandafter\def\csname R@cor/oneill/t/336/erased\endcsname{1.24}
\expandafter\def\csname R@cor/oneill/t/336/n\endcsname{52864}
\expandafter\def\csname R@cor/oneill/t/336/occ\endcsname{1.8}
\expandafter\def\csname R@cor/oneill/t/336/pnew/clean\endcsname{0.4}
\expandafter\def\csname R@cor/oneill/t/336/pnew/swap\endcsname{71}
\expandafter\def\csname R@cor/t/192/clean\endcsname{0.22}
\expandafter\def\csname R@cor/t/192/control\endcsname{0.22}
\expandafter\def\csname R@cor/t/192/erased\endcsname{1.10}
\expandafter\def\csname R@cor/t/192/n\endcsname{16693}
\expandafter\def\csname R@cor/t/192/occ\endcsname{1.3}
\expandafter\def\csname R@cor/t/192/pnew/clean\endcsname{0.5}
\expandafter\def\csname R@cor/t/192/pnew/swap\endcsname{55}
\expandafter\def\csname R@cor/t/336/clean\endcsname{0.19}
\expandafter\def\csname R@cor/t/336/control\endcsname{0.19}
\expandafter\def\csname R@cor/t/336/erased\endcsname{1.06}
\expandafter\def\csname R@cor/t/336/n\endcsname{22454}
\expandafter\def\csname R@cor/t/336/occ\endcsname{1.8}
\expandafter\def\csname R@cor/t/336/pnew/clean\endcsname{0.3}
\expandafter\def\csname R@cor/t/336/pnew/swap\endcsname{62}
\expandafter\def\csname R@gen/ae/acc\endcsname{99.94}
\expandafter\def\csname R@gen/ae/dist\endcsname{0.07}
\expandafter\def\csname R@gen/band/hi\endcsname{0.17}
\expandafter\def\csname R@gen/band/lo\endcsname{0.03}
\expandafter\def\csname R@gen/band/mean\endcsname{0.09}
\expandafter\def\csname R@gen/codes/18/fixed/exact\endcsname{0.0}
\expandafter\def\csname R@gen/codes/18/fixed/ham\endcsname{17.4}
\expandafter\def\csname R@gen/codes/18/tuned/exact\endcsname{0}
\expandafter\def\csname R@gen/codes/18/tuned/ham\endcsname{11.6}
\expandafter\def\csname R@gen/codes/192/fixed/exact\endcsname{0.0}
\expandafter\def\csname R@gen/codes/192/fixed/ham\endcsname{16.0}
\expandafter\def\csname R@gen/codes/192/tuned/exact\endcsname{14}
\expandafter\def\csname R@gen/codes/192/tuned/ham\endcsname{6.3}
\expandafter\def\csname R@gen/codes/336/fixed/exact\endcsname{0.2}
\expandafter\def\csname R@gen/codes/336/fixed/ham\endcsname{14.4}
\expandafter\def\csname R@gen/codes/336/tuned/exact\endcsname{32}
\expandafter\def\csname R@gen/codes/336/tuned/ham\endcsname{3.6}
\expandafter\def\csname R@gen/codes/48/fixed/exact\endcsname{0.0}
\expandafter\def\csname R@gen/codes/48/fixed/ham\endcsname{17.3}
\expandafter\def\csname R@gen/codes/48/tuned/exact\endcsname{0}
\expandafter\def\csname R@gen/codes/48/tuned/ham\endcsname{11.1}
\expandafter\def\csname R@gen/codes/6/fixed/exact\endcsname{0.0}
\expandafter\def\csname R@gen/codes/6/fixed/ham\endcsname{17.5}
\expandafter\def\csname R@gen/codes/6/tuned/exact\endcsname{0}
\expandafter\def\csname R@gen/codes/6/tuned/ham\endcsname{11.2}
\expandafter\def\csname R@gen/codes/96/fixed/exact\endcsname{0.0}
\expandafter\def\csname R@gen/codes/96/fixed/ham\endcsname{16.9}
\expandafter\def\csname R@gen/codes/96/tuned/exact\endcsname{1}
\expandafter\def\csname R@gen/codes/96/tuned/ham\endcsname{10.5}
\expandafter\def\csname R@gen/codes/fixed/ham/min\endcsname{14.4}
\expandafter\def\csname R@gen/codes/real/exact\endcsname{95.5}
\expandafter\def\csname R@gen/codes/real/ham\endcsname{0.40}
\expandafter\def\csname R@gen/codes/short/tuned/exact/max\endcsname{fewer than 0.1}
\expandafter\def\csname R@gen/codes/short/tuned/ham/min\endcsname{11.1}
\expandafter\def\csname R@gen/cut/first/hi\endcsname{0.17}
\expandafter\def\csname R@gen/cut/first/lo\endcsname{0.03}
\expandafter\def\csname R@gen/cut/first/nin\endcsname{0}
\expandafter\def\csname R@gen/cut/last/hi\endcsname{0.24}
\expandafter\def\csname R@gen/cut/last/lo\endcsname{0.04}
\expandafter\def\csname R@gen/cut/last/nin\endcsname{1}
\expandafter\def\csname R@gen/cut/random/hi\endcsname{0.17}
\expandafter\def\csname R@gen/cut/random/lo\endcsname{0.05}
\expandafter\def\csname R@gen/cut/random/nin\endcsname{0}
\expandafter\def\csname R@gen/fixed/latent/18/dist\endcsname{5.51}
\expandafter\def\csname R@gen/fixed/latent/18/struct\endcsname{0.00}
\expandafter\def\csname R@gen/fixed/latent/192/dist\endcsname{4.91}
\expandafter\def\csname R@gen/fixed/latent/192/struct\endcsname{0.00}
\expandafter\def\csname R@gen/fixed/latent/336/dist\endcsname{4.08}
\expandafter\def\csname R@gen/fixed/latent/336/struct\endcsname{0.01}
\expandafter\def\csname R@gen/fixed/latent/48/dist\endcsname{5.33}
\expandafter\def\csname R@gen/fixed/latent/48/struct\endcsname{0.00}
\expandafter\def\csname R@gen/fixed/latent/6/dist\endcsname{5.97}
\expandafter\def\csname R@gen/fixed/latent/6/struct\endcsname{0.00}
\expandafter\def\csname R@gen/fixed/latent/96/dist\endcsname{5.20}
\expandafter\def\csname R@gen/fixed/latent/96/struct\endcsname{0.00}
\expandafter\def\csname R@gen/fixed/token/18/dist\endcsname{2.33}
\expandafter\def\csname R@gen/fixed/token/18/struct\endcsname{0.00}
\expandafter\def\csname R@gen/fixed/token/192/dist\endcsname{1.92}
\expandafter\def\csname R@gen/fixed/token/192/struct\endcsname{0.06}
\expandafter\def\csname R@gen/fixed/token/336/dist\endcsname{1.69}
\expandafter\def\csname R@gen/fixed/token/336/struct\endcsname{0.09}
\expandafter\def\csname R@gen/fixed/token/48/dist\endcsname{2.21}
\expandafter\def\csname R@gen/fixed/token/48/struct\endcsname{0.00}
\expandafter\def\csname R@gen/fixed/token/6/dist\endcsname{2.83}
\expandafter\def\csname R@gen/fixed/token/6/struct\endcsname{0.00}
\expandafter\def\csname R@gen/fixed/token/96/dist\endcsname{1.78}
\expandafter\def\csname R@gen/fixed/token/96/struct\endcsname{0.01}
\expandafter\def\csname R@gen/latent/18/dens\endcsname{7.25}
\expandafter\def\csname R@gen/latent/18/dist\endcsname{1.19}
\expandafter\def\csname R@gen/latent/18/ent\endcsname{2.77}
\expandafter\def\csname R@gen/latent/18/mindist\endcsname{1.00}
\expandafter\def\csname R@gen/latent/18/n\endcsname{3}
\expandafter\def\csname R@gen/latent/18/rep\endcsname{0.48}
\expandafter\def\csname R@gen/latent/18/struct\endcsname{0.00}
\expandafter\def\csname R@gen/latent/18/tmin\endcsname{0.3}
\expandafter\def\csname R@gen/latent/192/dens\endcsname{6.93}
\expandafter\def\csname R@gen/latent/192/dist\endcsname{0.88}
\expandafter\def\csname R@gen/latent/192/ent\endcsname{2.50}
\expandafter\def\csname R@gen/latent/192/mindist\endcsname{0.81}
\expandafter\def\csname R@gen/latent/192/n\endcsname{3}
\expandafter\def\csname R@gen/latent/192/rep\endcsname{0.65}
\expandafter\def\csname R@gen/latent/192/struct\endcsname{0.12}
\expandafter\def\csname R@gen/latent/192/tmin\endcsname{0.3}
\expandafter\def\csname R@gen/latent/336/dens\endcsname{6.89}
\expandafter\def\csname R@gen/latent/336/dist\endcsname{0.68}
\expandafter\def\csname R@gen/latent/336/ent\endcsname{2.56}
\expandafter\def\csname R@gen/latent/336/mindist\endcsname{0.62}
\expandafter\def\csname R@gen/latent/336/n\endcsname{3}
\expandafter\def\csname R@gen/latent/336/rep\endcsname{0.67}
\expandafter\def\csname R@gen/latent/336/struct\endcsname{0.35}
\expandafter\def\csname R@gen/latent/336/tmin\endcsname{0.1}
\expandafter\def\csname R@gen/latent/48/dens\endcsname{7.20}
\expandafter\def\csname R@gen/latent/48/dist\endcsname{1.13}
\expandafter\def\csname R@gen/latent/48/ent\endcsname{2.75}
\expandafter\def\csname R@gen/latent/48/mindist\endcsname{0.97}
\expandafter\def\csname R@gen/latent/48/n\endcsname{3}
\expandafter\def\csname R@gen/latent/48/rep\endcsname{0.50}
\expandafter\def\csname R@gen/latent/48/struct\endcsname{0.01}
\expandafter\def\csname R@gen/latent/48/tmin\endcsname{0.3}
\expandafter\def\csname R@gen/latent/6/dens\endcsname{7.79}
\expandafter\def\csname R@gen/latent/6/dist\endcsname{1.21}
\expandafter\def\csname R@gen/latent/6/ent\endcsname{2.94}
\expandafter\def\csname R@gen/latent/6/mindist\endcsname{1.10}
\expandafter\def\csname R@gen/latent/6/n\endcsname{3}
\expandafter\def\csname R@gen/latent/6/rep\endcsname{0.48}
\expandafter\def\csname R@gen/latent/6/struct\endcsname{0.01}
\expandafter\def\csname R@gen/latent/6/tmin\endcsname{0.2}
\expandafter\def\csname R@gen/latent/96/dens\endcsname{7.19}
\expandafter\def\csname R@gen/latent/96/dist\endcsname{1.25}
\expandafter\def\csname R@gen/latent/96/ent\endcsname{2.52}
\expandafter\def\csname R@gen/latent/96/mindist\endcsname{1.19}
\expandafter\def\csname R@gen/latent/96/n\endcsname{3}
\expandafter\def\csname R@gen/latent/96/rep\endcsname{0.55}
\expandafter\def\csname R@gen/latent/96/struct\endcsname{0.02}
\expandafter\def\csname R@gen/latent/96/tmin\endcsname{0.4}
\expandafter\def\csname R@gen/latent/short/struct/max\endcsname{0.01}
\expandafter\def\csname R@gen/longtunes\endcsname{12}
\expandafter\def\csname R@gen/min/ctx\endcsname{192}
\expandafter\def\csname R@gen/min/dist\endcsname{0.19}
\expandafter\def\csname R@gen/min/kind\endcsname{token}
\expandafter\def\csname R@gen/nsets\endcsname{36}
\expandafter\def\csname R@gen/ref/dens\endcsname{6.95}
\expandafter\def\csname R@gen/ref/ent\endcsname{3.09}
\expandafter\def\csname R@gen/ref/rep\endcsname{0.69}
\expandafter\def\csname R@gen/struct/hi\endcsname{0.52}
\expandafter\def\csname R@gen/struct/lo\endcsname{0.48}
\expandafter\def\csname R@gen/struct/real\endcsname{0.50}
\expandafter\def\csname R@gen/token/18/dens\endcsname{5.83}
\expandafter\def\csname R@gen/token/18/dist\endcsname{1.66}
\expandafter\def\csname R@gen/token/18/ent\endcsname{3.90}
\expandafter\def\csname R@gen/token/18/mindist\endcsname{1.61}
\expandafter\def\csname R@gen/token/18/n\endcsname{3}
\expandafter\def\csname R@gen/token/18/rep\endcsname{0.84}
\expandafter\def\csname R@gen/token/18/struct\endcsname{0.01}
\expandafter\def\csname R@gen/token/18/tmin\endcsname{0.8}
\expandafter\def\csname R@gen/token/192/dens\endcsname{6.81}
\expandafter\def\csname R@gen/token/192/dist\endcsname{0.25}
\expandafter\def\csname R@gen/token/192/ent\endcsname{2.91}
\expandafter\def\csname R@gen/token/192/mindist\endcsname{0.19}
\expandafter\def\csname R@gen/token/192/n\endcsname{3}
\expandafter\def\csname R@gen/token/192/rep\endcsname{0.70}
\expandafter\def\csname R@gen/token/192/struct\endcsname{0.41}
\expandafter\def\csname R@gen/token/192/tmin\endcsname{0.8}
\expandafter\def\csname R@gen/token/336/dens\endcsname{7.32}
\expandafter\def\csname R@gen/token/336/dist\endcsname{0.29}
\expandafter\def\csname R@gen/token/336/ent\endcsname{3.01}
\expandafter\def\csname R@gen/token/336/mindist\endcsname{0.28}
\expandafter\def\csname R@gen/token/336/n\endcsname{3}
\expandafter\def\csname R@gen/token/336/rep\endcsname{0.69}
\expandafter\def\csname R@gen/token/336/struct\endcsname{0.41}
\expandafter\def\csname R@gen/token/336/tmin\endcsname{0.8}
\expandafter\def\csname R@gen/token/48/dens\endcsname{7.35}
\expandafter\def\csname R@gen/token/48/dist\endcsname{1.37}
\expandafter\def\csname R@gen/token/48/ent\endcsname{4.03}
\expandafter\def\csname R@gen/token/48/mindist\endcsname{1.34}
\expandafter\def\csname R@gen/token/48/n\endcsname{3}
\expandafter\def\csname R@gen/token/48/rep\endcsname{0.77}
\expandafter\def\csname R@gen/token/48/struct\endcsname{0.00}
\expandafter\def\csname R@gen/token/48/tmin\endcsname{0.9}
\expandafter\def\csname R@gen/token/6/dens\endcsname{6.51}
\expandafter\def\csname R@gen/token/6/dist\endcsname{1.49}
\expandafter\def\csname R@gen/token/6/ent\endcsname{3.88}
\expandafter\def\csname R@gen/token/6/mindist\endcsname{1.39}
\expandafter\def\csname R@gen/token/6/n\endcsname{3}
\expandafter\def\csname R@gen/token/6/rep\endcsname{0.82}
\expandafter\def\csname R@gen/token/6/struct\endcsname{0.01}
\expandafter\def\csname R@gen/token/6/tmin\endcsname{0.7}
\expandafter\def\csname R@gen/token/96/dens\endcsname{6.55}
\expandafter\def\csname R@gen/token/96/dist\endcsname{1.09}
\expandafter\def\csname R@gen/token/96/ent\endcsname{3.62}
\expandafter\def\csname R@gen/token/96/mindist\endcsname{0.29}
\expandafter\def\csname R@gen/token/96/n\endcsname{3}
\expandafter\def\csname R@gen/token/96/rep\endcsname{0.79}
\expandafter\def\csname R@gen/token/96/struct\endcsname{0.06}
\expandafter\def\csname R@gen/token/96/tmin\endcsname{0.8}
\expandafter\def\csname R@maes/abl/t/repl/18\endcsname{3.262}
\expandafter\def\csname R@maes/abl/t/repl/18/none\endcsname{3.272}
\expandafter\def\csname R@maes/abl/t/repl/18/repeat\endcsname{1.891}
\expandafter\def\csname R@maes/abl/t/repl/192\endcsname{3.002}
\expandafter\def\csname R@maes/abl/t/repl/192/none\endcsname{3.013}
\expandafter\def\csname R@maes/abl/t/repl/192/repeat\endcsname{1.517}
\expandafter\def\csname R@maes/abl/t/repl/48\endcsname{3.081}
\expandafter\def\csname R@maes/abl/t/repl/48/none\endcsname{3.092}
\expandafter\def\csname R@maes/abl/t/repl/48/repeat\endcsname{1.670}
\expandafter\def\csname R@maes/abl/t/repl/6\endcsname{3.682}
\expandafter\def\csname R@maes/abl/t/repl/6/none\endcsname{3.692}
\expandafter\def\csname R@maes/abl/t/repl/6/repeat\endcsname{2.288}
\expandafter\def\csname R@maes/abl/t/repl/96\endcsname{3.025}
\expandafter\def\csname R@maes/abl/t/repl/96/none\endcsname{3.036}
\expandafter\def\csname R@maes/abl/t/repl/96/repeat\endcsname{1.578}
\expandafter\def\csname R@maes/abl/t/sweep/18\endcsname{3.174}
\expandafter\def\csname R@maes/abl/t/sweep/192\endcsname{3.012}
\expandafter\def\csname R@maes/abl/t/sweep/336\endcsname{2.985}
\expandafter\def\csname R@maes/abl/t/sweep/48\endcsname{3.093}
\expandafter\def\csname R@maes/abl/t/sweep/6\endcsname{3.279}
\expandafter\def\csname R@maes/abl/t/sweep/96\endcsname{3.036}
\expandafter\def\csname R@maes/abl/t/trunc/18\endcsname{3.221}
\expandafter\def\csname R@maes/abl/t/trunc/18/none\endcsname{3.232}
\expandafter\def\csname R@maes/abl/t/trunc/18/repeat\endcsname{1.740}
\expandafter\def\csname R@maes/abl/t/trunc/192\endcsname{2.998}
\expandafter\def\csname R@maes/abl/t/trunc/192/none\endcsname{3.010}
\expandafter\def\csname R@maes/abl/t/trunc/192/repeat\endcsname{1.495}
\expandafter\def\csname R@maes/abl/t/trunc/336\endcsname{2.985}
\expandafter\def\csname R@maes/abl/t/trunc/336/none\endcsname{2.996}
\expandafter\def\csname R@maes/abl/t/trunc/336/repeat\endcsname{1.444}
\expandafter\def\csname R@maes/abl/t/trunc/48\endcsname{3.062}
\expandafter\def\csname R@maes/abl/t/trunc/48/none\endcsname{3.073}
\expandafter\def\csname R@maes/abl/t/trunc/48/repeat\endcsname{1.593}
\expandafter\def\csname R@maes/abl/t/trunc/6\endcsname{3.575}
\expandafter\def\csname R@maes/abl/t/trunc/6/none\endcsname{3.587}
\expandafter\def\csname R@maes/abl/t/trunc/6/repeat\endcsname{1.912}
\expandafter\def\csname R@maes/abl/t/trunc/96\endcsname{3.016}
\expandafter\def\csname R@maes/abl/t/trunc/96/none\endcsname{3.027}
\expandafter\def\csname R@maes/abl/t/trunc/96/repeat\endcsname{1.546}
\expandafter\def\csname R@maes/abl/targets\endcsname{40{,}068}
\expandafter\def\csname R@maes/ae/acc\endcsname{99.999}
\expandafter\def\csname R@maes/align/192/aligned\endcsname{0.74}
\expandafter\def\csname R@maes/align/192/misaligned\endcsname{0.66}
\expandafter\def\csname R@maes/align/192/share\endcsname{30}
\expandafter\def\csname R@maes/align/336/aligned\endcsname{0.72}
\expandafter\def\csname R@maes/align/336/misaligned\endcsname{0.62}
\expandafter\def\csname R@maes/align/336/share\endcsname{23}
\expandafter\def\csname R@maes/align/96/aligned\endcsname{0.85}
\expandafter\def\csname R@maes/align/96/misaligned\endcsname{0.69}
\expandafter\def\csname R@maes/align/96/share\endcsname{25}
\expandafter\def\csname R@maes/aligned/1-32\endcsname{20}
\expandafter\def\csname R@maes/aligned/177-320\endcsname{15}
\expandafter\def\csname R@maes/aligned/33-80\endcsname{22}
\expandafter\def\csname R@maes/aligned/81-176\endcsname{30}
\expandafter\def\csname R@maes/aligned/all\endcsname{21}
\expandafter\def\csname R@maes/boot/l/18-48\endcsname{0.0024}
\expandafter\def\csname R@maes/boot/l/18-48/hi\endcsname{0.0031}
\expandafter\def\csname R@maes/boot/l/18-48/lo\endcsname{0.0017}
\expandafter\def\csname R@maes/boot/l/18-6\endcsname{-0.0056}
\expandafter\def\csname R@maes/boot/l/18-6/hi\endcsname{-0.0047}
\expandafter\def\csname R@maes/boot/l/18-6/lo\endcsname{-0.0064}
\expandafter\def\csname R@maes/boot/l/192-336\endcsname{-0.0001}
\expandafter\def\csname R@maes/boot/l/192-336/hi\endcsname{0.0003}
\expandafter\def\csname R@maes/boot/l/192-336/lo\endcsname{-0.0006}
\expandafter\def\csname R@maes/boot/l/192-96\endcsname{-0.0005}
\expandafter\def\csname R@maes/boot/l/192-96/hi\endcsname{-0.0001}
\expandafter\def\csname R@maes/boot/l/192-96/lo\endcsname{-0.0010}
\expandafter\def\csname R@maes/boot/l/336-192\endcsname{0.0001}
\expandafter\def\csname R@maes/boot/l/336-192/hi\endcsname{0.0006}
\expandafter\def\csname R@maes/boot/l/336-192/lo\endcsname{-0.0003}
\expandafter\def\csname R@maes/boot/l/336-48\endcsname{-0.0022}
\expandafter\def\csname R@maes/boot/l/336-48/hi\endcsname{-0.0016}
\expandafter\def\csname R@maes/boot/l/336-48/lo\endcsname{-0.0028}
\expandafter\def\csname R@maes/boot/l/336-6\endcsname{-0.0102}
\expandafter\def\csname R@maes/boot/l/336-6/hi\endcsname{-0.0090}
\expandafter\def\csname R@maes/boot/l/336-6/lo\endcsname{-0.0114}
\expandafter\def\csname R@maes/boot/l/336-96\endcsname{-0.0004}
\expandafter\def\csname R@maes/boot/l/336-96/hi\endcsname{0.0001}
\expandafter\def\csname R@maes/boot/l/336-96/lo\endcsname{-0.0009}
\expandafter\def\csname R@maes/boot/l/48-18\endcsname{-0.0024}
\expandafter\def\csname R@maes/boot/l/48-18/hi\endcsname{-0.0017}
\expandafter\def\csname R@maes/boot/l/48-18/lo\endcsname{-0.0031}
\expandafter\def\csname R@maes/boot/l/48-336\endcsname{0.0022}
\expandafter\def\csname R@maes/boot/l/48-336/hi\endcsname{0.0028}
\expandafter\def\csname R@maes/boot/l/48-336/lo\endcsname{0.0016}
\expandafter\def\csname R@maes/boot/l/48-96\endcsname{0.0018}
\expandafter\def\csname R@maes/boot/l/48-96/hi\endcsname{0.0023}
\expandafter\def\csname R@maes/boot/l/48-96/lo\endcsname{0.0013}
\expandafter\def\csname R@maes/boot/l/6-18\endcsname{0.0056}
\expandafter\def\csname R@maes/boot/l/6-18/hi\endcsname{0.0064}
\expandafter\def\csname R@maes/boot/l/6-18/lo\endcsname{0.0047}
\expandafter\def\csname R@maes/boot/l/6-336\endcsname{0.0102}
\expandafter\def\csname R@maes/boot/l/6-336/hi\endcsname{0.0114}
\expandafter\def\csname R@maes/boot/l/6-336/lo\endcsname{0.0090}
\expandafter\def\csname R@maes/boot/l/96-192\endcsname{0.0005}
\expandafter\def\csname R@maes/boot/l/96-192/hi\endcsname{0.0010}
\expandafter\def\csname R@maes/boot/l/96-192/lo\endcsname{0.0001}
\expandafter\def\csname R@maes/boot/l/96-336\endcsname{0.0004}
\expandafter\def\csname R@maes/boot/l/96-336/hi\endcsname{0.0009}
\expandafter\def\csname R@maes/boot/l/96-336/lo\endcsname{-0.0001}
\expandafter\def\csname R@maes/boot/l/96-48\endcsname{-0.0018}
\expandafter\def\csname R@maes/boot/l/96-48/hi\endcsname{-0.0013}
\expandafter\def\csname R@maes/boot/l/96-48/lo\endcsname{-0.0023}
\expandafter\def\csname R@maes/boot/t/18-48\endcsname{0.080}
\expandafter\def\csname R@maes/boot/t/18-48/hi\endcsname{0.088}
\expandafter\def\csname R@maes/boot/t/18-48/lo\endcsname{0.072}
\expandafter\def\csname R@maes/boot/t/18-6\endcsname{-0.106}
\expandafter\def\csname R@maes/boot/t/18-6/hi\endcsname{-0.099}
\expandafter\def\csname R@maes/boot/t/18-6/lo\endcsname{-0.113}
\expandafter\def\csname R@maes/boot/t/192-336\endcsname{0.026}
\expandafter\def\csname R@maes/boot/t/192-336/hi\endcsname{0.031}
\expandafter\def\csname R@maes/boot/t/192-336/lo\endcsname{0.021}
\expandafter\def\csname R@maes/boot/t/192-96\endcsname{-0.028}
\expandafter\def\csname R@maes/boot/t/192-96/hi\endcsname{-0.023}
\expandafter\def\csname R@maes/boot/t/192-96/lo\endcsname{-0.032}
\expandafter\def\csname R@maes/boot/t/336-192\endcsname{-0.026}
\expandafter\def\csname R@maes/boot/t/336-192/hi\endcsname{-0.021}
\expandafter\def\csname R@maes/boot/t/336-192/lo\endcsname{-0.031}
\expandafter\def\csname R@maes/boot/t/336-48\endcsname{-0.110}
\expandafter\def\csname R@maes/boot/t/336-48/hi\endcsname{-0.099}
\expandafter\def\csname R@maes/boot/t/336-48/lo\endcsname{-0.123}
\expandafter\def\csname R@maes/boot/t/336-6\endcsname{-0.296}
\expandafter\def\csname R@maes/boot/t/336-6/hi\endcsname{-0.276}
\expandafter\def\csname R@maes/boot/t/336-6/lo\endcsname{-0.318}
\expandafter\def\csname R@maes/boot/t/336-96\endcsname{-0.054}
\expandafter\def\csname R@maes/boot/t/336-96/hi\endcsname{-0.047}
\expandafter\def\csname R@maes/boot/t/336-96/lo\endcsname{-0.061}
\expandafter\def\csname R@maes/boot/t/48-18\endcsname{-0.080}
\expandafter\def\csname R@maes/boot/t/48-18/hi\endcsname{-0.072}
\expandafter\def\csname R@maes/boot/t/48-18/lo\endcsname{-0.088}
\expandafter\def\csname R@maes/boot/t/48-336\endcsname{0.110}
\expandafter\def\csname R@maes/boot/t/48-336/hi\endcsname{0.123}
\expandafter\def\csname R@maes/boot/t/48-336/lo\endcsname{0.099}
\expandafter\def\csname R@maes/boot/t/48-96\endcsname{0.057}
\expandafter\def\csname R@maes/boot/t/48-96/hi\endcsname{0.064}
\expandafter\def\csname R@maes/boot/t/48-96/lo\endcsname{0.050}
\expandafter\def\csname R@maes/boot/t/6-18\endcsname{0.106}
\expandafter\def\csname R@maes/boot/t/6-18/hi\endcsname{0.113}
\expandafter\def\csname R@maes/boot/t/6-18/lo\endcsname{0.099}
\expandafter\def\csname R@maes/boot/t/6-336\endcsname{0.296}
\expandafter\def\csname R@maes/boot/t/6-336/hi\endcsname{0.318}
\expandafter\def\csname R@maes/boot/t/6-336/lo\endcsname{0.276}
\expandafter\def\csname R@maes/boot/t/96-192\endcsname{0.028}
\expandafter\def\csname R@maes/boot/t/96-192/hi\endcsname{0.032}
\expandafter\def\csname R@maes/boot/t/96-192/lo\endcsname{0.023}
\expandafter\def\csname R@maes/boot/t/96-336\endcsname{0.054}
\expandafter\def\csname R@maes/boot/t/96-336/hi\endcsname{0.061}
\expandafter\def\csname R@maes/boot/t/96-336/lo\endcsname{0.047}
\expandafter\def\csname R@maes/boot/t/96-48\endcsname{-0.057}
\expandafter\def\csname R@maes/boot/t/96-48/hi\endcsname{-0.050}
\expandafter\def\csname R@maes/boot/t/96-48/lo\endcsname{-0.064}
\expandafter\def\csname R@maes/clamped\endcsname{5.6}
\expandafter\def\csname R@maes/copy/s/1-32\endcsname{15}
\expandafter\def\csname R@maes/copy/s/177-320\endcsname{35}
\expandafter\def\csname R@maes/copy/s/33-80\endcsname{20}
\expandafter\def\csname R@maes/copy/s/81-176\endcsname{40}
\expandafter\def\csname R@maes/copy/s/all\endcsname{29}
\expandafter\def\csname R@maes/copy/t/1-32\endcsname{75}
\expandafter\def\csname R@maes/copy/t/177-320\endcsname{83}
\expandafter\def\csname R@maes/copy/t/33-80\endcsname{81}
\expandafter\def\csname R@maes/copy/t/81-176\endcsname{80}
\expandafter\def\csname R@maes/copy/t/all\endcsname{81}
\expandafter\def\csname R@maes/copybase/16\endcsname{3.277}
\expandafter\def\csname R@maes/copybase/16/gain\endcsname{2}
\expandafter\def\csname R@maes/copybase/16/matched\endcsname{1}
\expandafter\def\csname R@maes/copybase/backoff\endcsname{3.249}
\expandafter\def\csname R@maes/copybase/backoff/gain\endcsname{11}
\expandafter\def\csname R@maes/copybase/backoff/matched\endcsname{4}
\expandafter\def\csname R@maes/copybase/base\endcsname{3.283}
\expandafter\def\csname R@maes/copybase/m/bits_T336\endcsname{1.92}
\expandafter\def\csname R@maes/copybase/m/bits_T6\endcsname{2.47}
\expandafter\def\csname R@maes/copybase/m/bits_copy\endcsname{1.70}
\expandafter\def\csname R@maes/copybase/m/copy\endcsname{11}
\expandafter\def\csname R@maes/copybase/m/t336\endcsname{8}
\expandafter\def\csname R@maes/groups\endcsname{856}
\expandafter\def\csname R@maes/h32/copy\endcsname{77}
\expandafter\def\csname R@maes/h32/redshare/l\endcsname{0}
\expandafter\def\csname R@maes/h32/redshare/t\endcsname{0}
\expandafter\def\csname R@maes/h32/share\endcsname{0}
\expandafter\def\csname R@maes/h8/copy\endcsname{72}
\expandafter\def\csname R@maes/h8/redshare/l\endcsname{9}
\expandafter\def\csname R@maes/h8/redshare/t\endcsname{8}
\expandafter\def\csname R@maes/h8/share\endcsname{4}
\expandafter\def\csname R@maes/inview/18\endcsname{0.0}
\expandafter\def\csname R@maes/inview/192\endcsname{0.5}
\expandafter\def\csname R@maes/inview/336\endcsname{0.8}
\expandafter\def\csname R@maes/inview/48\endcsname{0.1}
\expandafter\def\csname R@maes/inview/6\endcsname{0.0}
\expandafter\def\csname R@maes/inview/96\endcsname{0.3}
\expandafter\def\csname R@maes/lag/l/18/1-32\endcsname{0.77}
\expandafter\def\csname R@maes/lag/l/18/177-320\endcsname{0.73}
\expandafter\def\csname R@maes/lag/l/18/33-80\endcsname{0.81}
\expandafter\def\csname R@maes/lag/l/18/81-176\endcsname{0.79}
\expandafter\def\csname R@maes/lag/l/18/held\endcsname{0.58}
\expandafter\def\csname R@maes/lag/l/18/none\endcsname{0.89}
\expandafter\def\csname R@maes/lag/l/192/1-32\endcsname{0.75}
\expandafter\def\csname R@maes/lag/l/192/177-320\endcsname{0.71}
\expandafter\def\csname R@maes/lag/l/192/33-80\endcsname{0.78}
\expandafter\def\csname R@maes/lag/l/192/81-176\endcsname{0.77}
\expandafter\def\csname R@maes/lag/l/192/held\endcsname{0.57}
\expandafter\def\csname R@maes/lag/l/192/none\endcsname{0.89}
\expandafter\def\csname R@maes/lag/l/336/1-32\endcsname{0.76}
\expandafter\def\csname R@maes/lag/l/336/177-320\endcsname{0.71}
\expandafter\def\csname R@maes/lag/l/336/33-80\endcsname{0.78}
\expandafter\def\csname R@maes/lag/l/336/81-176\endcsname{0.78}
\expandafter\def\csname R@maes/lag/l/336/held\endcsname{0.57}
\expandafter\def\csname R@maes/lag/l/336/none\endcsname{0.89}
\expandafter\def\csname R@maes/lag/l/48/1-32\endcsname{0.75}
\expandafter\def\csname R@maes/lag/l/48/177-320\endcsname{0.73}
\expandafter\def\csname R@maes/lag/l/48/33-80\endcsname{0.79}
\expandafter\def\csname R@maes/lag/l/48/81-176\endcsname{0.78}
\expandafter\def\csname R@maes/lag/l/48/held\endcsname{0.57}
\expandafter\def\csname R@maes/lag/l/48/none\endcsname{0.89}
\expandafter\def\csname R@maes/lag/l/6/1-32\endcsname{0.79}
\expandafter\def\csname R@maes/lag/l/6/177-320\endcsname{0.74}
\expandafter\def\csname R@maes/lag/l/6/33-80\endcsname{0.81}
\expandafter\def\csname R@maes/lag/l/6/81-176\endcsname{0.80}
\expandafter\def\csname R@maes/lag/l/6/held\endcsname{0.60}
\expandafter\def\csname R@maes/lag/l/6/none\endcsname{0.90}
\expandafter\def\csname R@maes/lag/l/96/1-32\endcsname{0.75}
\expandafter\def\csname R@maes/lag/l/96/177-320\endcsname{0.72}
\expandafter\def\csname R@maes/lag/l/96/33-80\endcsname{0.78}
\expandafter\def\csname R@maes/lag/l/96/81-176\endcsname{0.78}
\expandafter\def\csname R@maes/lag/l/96/held\endcsname{0.57}
\expandafter\def\csname R@maes/lag/l/96/none\endcsname{0.89}
\expandafter\def\csname R@maes/lag/t/18/1-32\endcsname{1.87}
\expandafter\def\csname R@maes/lag/t/18/177-320\endcsname{1.64}
\expandafter\def\csname R@maes/lag/t/18/33-80\endcsname{2.05}
\expandafter\def\csname R@maes/lag/t/18/81-176\endcsname{2.01}
\expandafter\def\csname R@maes/lag/t/18/held\endcsname{1.03}
\expandafter\def\csname R@maes/lag/t/18/none\endcsname{3.24}
\expandafter\def\csname R@maes/lag/t/192/1-32\endcsname{1.68}
\expandafter\def\csname R@maes/lag/t/192/177-320\endcsname{1.56}
\expandafter\def\csname R@maes/lag/t/192/33-80\endcsname{1.72}
\expandafter\def\csname R@maes/lag/t/192/81-176\endcsname{1.70}
\expandafter\def\csname R@maes/lag/t/192/held\endcsname{0.99}
\expandafter\def\csname R@maes/lag/t/192/none\endcsname{3.07}
\expandafter\def\csname R@maes/lag/t/336/1-32\endcsname{1.64}
\expandafter\def\csname R@maes/lag/t/336/177-320\endcsname{1.35}
\expandafter\def\csname R@maes/lag/t/336/33-80\endcsname{1.57}
\expandafter\def\csname R@maes/lag/t/336/81-176\endcsname{1.63}
\expandafter\def\csname R@maes/lag/t/336/held\endcsname{0.99}
\expandafter\def\csname R@maes/lag/t/336/none\endcsname{3.05}
\expandafter\def\csname R@maes/lag/t/48/1-32\endcsname{1.66}
\expandafter\def\csname R@maes/lag/t/48/177-320\endcsname{1.58}
\expandafter\def\csname R@maes/lag/t/48/33-80\endcsname{1.96}
\expandafter\def\csname R@maes/lag/t/48/81-176\endcsname{1.94}
\expandafter\def\csname R@maes/lag/t/48/held\endcsname{1.00}
\expandafter\def\csname R@maes/lag/t/48/none\endcsname{3.16}
\expandafter\def\csname R@maes/lag/t/6/1-32\endcsname{1.93}
\expandafter\def\csname R@maes/lag/t/6/177-320\endcsname{1.67}
\expandafter\def\csname R@maes/lag/t/6/33-80\endcsname{2.13}
\expandafter\def\csname R@maes/lag/t/6/81-176\endcsname{2.06}
\expandafter\def\csname R@maes/lag/t/6/held\endcsname{1.06}
\expandafter\def\csname R@maes/lag/t/6/none\endcsname{3.35}
\expandafter\def\csname R@maes/lag/t/96/1-32\endcsname{1.72}
\expandafter\def\csname R@maes/lag/t/96/177-320\endcsname{1.56}
\expandafter\def\csname R@maes/lag/t/96/33-80\endcsname{1.76}
\expandafter\def\csname R@maes/lag/t/96/81-176\endcsname{1.86}
\expandafter\def\csname R@maes/lag/t/96/held\endcsname{0.99}
\expandafter\def\csname R@maes/lag/t/96/none\endcsname{3.10}
\expandafter\def\csname R@maes/lat/0\endcsname{0.978}
\expandafter\def\csname R@maes/lat/0/n\endcsname{1}
\expandafter\def\csname R@maes/lat/0/pertoken\endcsname{10.43}
\expandafter\def\csname R@maes/lat/18\endcsname{0.881}
\expandafter\def\csname R@maes/lat/18/ep/max\endcsname{9}
\expandafter\def\csname R@maes/lat/18/ep/min\endcsname{8}
\expandafter\def\csname R@maes/lat/18/n\endcsname{3}
\expandafter\def\csname R@maes/lat/18/pertoken\endcsname{9.40}
\expandafter\def\csname R@maes/lat/18/sd\endcsname{0.000}
\expandafter\def\csname R@maes/lat/192\endcsname{0.877}
\expandafter\def\csname R@maes/lat/192/ep/max\endcsname{7}
\expandafter\def\csname R@maes/lat/192/ep/min\endcsname{7}
\expandafter\def\csname R@maes/lat/192/n\endcsname{3}
\expandafter\def\csname R@maes/lat/192/pertoken\endcsname{9.35}
\expandafter\def\csname R@maes/lat/192/sd\endcsname{0.000}
\expandafter\def\csname R@maes/lat/336\endcsname{0.877}
\expandafter\def\csname R@maes/lat/336/ep/max\endcsname{7}
\expandafter\def\csname R@maes/lat/336/ep/min\endcsname{6}
\expandafter\def\csname R@maes/lat/336/n\endcsname{3}
\expandafter\def\csname R@maes/lat/336/pertoken\endcsname{9.35}
\expandafter\def\csname R@maes/lat/336/sd\endcsname{0.000}
\expandafter\def\csname R@maes/lat/48\endcsname{0.879}
\expandafter\def\csname R@maes/lat/48/ep/max\endcsname{8}
\expandafter\def\csname R@maes/lat/48/ep/min\endcsname{6}
\expandafter\def\csname R@maes/lat/48/n\endcsname{3}
\expandafter\def\csname R@maes/lat/48/pertoken\endcsname{9.38}
\expandafter\def\csname R@maes/lat/48/sd\endcsname{0.000}
\expandafter\def\csname R@maes/lat/6\endcsname{0.887}
\expandafter\def\csname R@maes/lat/6/ep/max\endcsname{14}
\expandafter\def\csname R@maes/lat/6/ep/min\endcsname{9}
\expandafter\def\csname R@maes/lat/6/n\endcsname{3}
\expandafter\def\csname R@maes/lat/6/pertoken\endcsname{9.46}
\expandafter\def\csname R@maes/lat/6/sd\endcsname{0.000}
\expandafter\def\csname R@maes/lat/96\endcsname{0.877}
\expandafter\def\csname R@maes/lat/96/ep/max\endcsname{7}
\expandafter\def\csname R@maes/lat/96/ep/min\endcsname{5}
\expandafter\def\csname R@maes/lat/96/n\endcsname{3}
\expandafter\def\csname R@maes/lat/96/pertoken\endcsname{9.36}
\expandafter\def\csname R@maes/lat/96/sd\endcsname{0.000}
\expandafter\def\csname R@maes/lat/drop\endcsname{1}
\expandafter\def\csname R@maes/lat/ep/max\endcsname{14}
\expandafter\def\csname R@maes/lat/maxsd\endcsname{0.000}
\expandafter\def\csname R@maes/leak/test/verbatim\endcsname{0.2}
\expandafter\def\csname R@maes/lenratio\endcsname{1.73}
\expandafter\def\csname R@maes/longep/max\endcsname{15}
\expandafter\def\csname R@maes/longep/min\endcsname{6}
\expandafter\def\csname R@maes/moved\endcsname{0}
\expandafter\def\csname R@maes/pieces/all\endcsname{1276}
\expandafter\def\csname R@maes/pieces/test\endcsname{177}
\expandafter\def\csname R@maes/pieces/testwin\endcsname{177}
\expandafter\def\csname R@maes/pieces/train\endcsname{962}
\expandafter\def\csname R@maes/pieces/val\endcsname{137}
\expandafter\def\csname R@maes/pitchlo\endcsname{48}
\expandafter\def\csname R@maes/reached/l/18\endcsname{55}
\expandafter\def\csname R@maes/reached/l/192\endcsname{101}
\expandafter\def\csname R@maes/reached/l/336\endcsname{100}
\expandafter\def\csname R@maes/reached/l/48\endcsname{79}
\expandafter\def\csname R@maes/reached/l/6\endcsname{0}
\expandafter\def\csname R@maes/reached/l/96\endcsname{96}
\expandafter\def\csname R@maes/reached/t/18\endcsname{36}
\expandafter\def\csname R@maes/reached/t/192\endcsname{91}
\expandafter\def\csname R@maes/reached/t/336\endcsname{100}
\expandafter\def\csname R@maes/reached/t/48\endcsname{63}
\expandafter\def\csname R@maes/reached/t/6\endcsname{0}
\expandafter\def\csname R@maes/reached/t/96\endcsname{82}
\expandafter\def\csname R@maes/redshare/l/none\endcsname{91}
\expandafter\def\csname R@maes/redshare/l/repeat\endcsname{2}
\expandafter\def\csname R@maes/redshare/t/none\endcsname{98}
\expandafter\def\csname R@maes/redshare/t/none1\endcsname{98.4}
\expandafter\def\csname R@maes/redshare/t/repeat\endcsname{1}
\expandafter\def\csname R@maes/rest\endcsname{14.0}
\expandafter\def\csname R@maes/share/s/1-32\endcsname{0.1}
\expandafter\def\csname R@maes/share/s/177-320\endcsname{0.3}
\expandafter\def\csname R@maes/share/s/33-80\endcsname{0.2}
\expandafter\def\csname R@maes/share/s/81-176\endcsname{0.2}
\expandafter\def\csname R@maes/share/s/held\endcsname{2.4}
\expandafter\def\csname R@maes/share/s/none\endcsname{96.8}
\expandafter\def\csname R@maes/share/s/repeat\endcsname{1}
\expandafter\def\csname R@maes/share/t/1-32\endcsname{0.1}
\expandafter\def\csname R@maes/share/t/177-320\endcsname{0.2}
\expandafter\def\csname R@maes/share/t/33-80\endcsname{0.2}
\expandafter\def\csname R@maes/share/t/81-176\endcsname{0.2}
\expandafter\def\csname R@maes/share/t/held\endcsname{2.3}
\expandafter\def\csname R@maes/share/t/none\endcsname{96.9}
\expandafter\def\csname R@maes/share/t/repeat\endcsname{1}
\expandafter\def\csname R@maes/share/t/repeat2\endcsname{0.76}
\expandafter\def\csname R@maes/targets\endcsname{144}
\expandafter\def\csname R@maes/tok/0\endcsname{5.319}
\expandafter\def\csname R@maes/tok/0/n\endcsname{1}
\expandafter\def\csname R@maes/tok/18\endcsname{3.177}
\expandafter\def\csname R@maes/tok/18/ep/max\endcsname{12}
\expandafter\def\csname R@maes/tok/18/ep/min\endcsname{11}
\expandafter\def\csname R@maes/tok/18/n\endcsname{3}
\expandafter\def\csname R@maes/tok/18/sd\endcsname{0.002}
\expandafter\def\csname R@maes/tok/192\endcsname{3.013}
\expandafter\def\csname R@maes/tok/192/ep/max\endcsname{11}
\expandafter\def\csname R@maes/tok/192/ep/min\endcsname{10}
\expandafter\def\csname R@maes/tok/192/n\endcsname{3}
\expandafter\def\csname R@maes/tok/192/sd\endcsname{0.005}
\expandafter\def\csname R@maes/tok/336\endcsname{2.987}
\expandafter\def\csname R@maes/tok/336/ep/max\endcsname{15}
\expandafter\def\csname R@maes/tok/336/ep/min\endcsname{12}
\expandafter\def\csname R@maes/tok/336/n\endcsname{3}
\expandafter\def\csname R@maes/tok/336/sd\endcsname{0.005}
\expandafter\def\csname R@maes/tok/48\endcsname{3.097}
\expandafter\def\csname R@maes/tok/48/ep/max\endcsname{13}
\expandafter\def\csname R@maes/tok/48/ep/min\endcsname{11}
\expandafter\def\csname R@maes/tok/48/n\endcsname{3}
\expandafter\def\csname R@maes/tok/48/sd\endcsname{0.006}
\expandafter\def\csname R@maes/tok/6\endcsname{3.283}
\expandafter\def\csname R@maes/tok/6/ep/max\endcsname{14}
\expandafter\def\csname R@maes/tok/6/ep/min\endcsname{9}
\expandafter\def\csname R@maes/tok/6/n\endcsname{3}
\expandafter\def\csname R@maes/tok/6/sd\endcsname{0.002}
\expandafter\def\csname R@maes/tok/96\endcsname{3.040}
\expandafter\def\csname R@maes/tok/96/ep/max\endcsname{11}
\expandafter\def\csname R@maes/tok/96/ep/min\endcsname{10}
\expandafter\def\csname R@maes/tok/96/n\endcsname{3}
\expandafter\def\csname R@maes/tok/96/sd\endcsname{0.009}
\expandafter\def\csname R@maes/tok/drop\endcsname{9}
\expandafter\def\csname R@maes/tok/ep/max\endcsname{15}
\expandafter\def\csname R@maes/tok/maxsd\endcsname{0.009}
\expandafter\def\csname R@maes/tokens/test\endcsname{575{,}427}
\expandafter\def\csname R@maes/tokens/train\endcsname{4{,}586{,}280}
\expandafter\def\csname R@maes/tokens/val\endcsname{559{,}582}
\expandafter\def\csname R@maes/trans/copy\endcsname{75}
\expandafter\def\csname R@maes/trans/other/336\endcsname{2.90}
\expandafter\def\csname R@maes/trans/other/6\endcsname{3.21}
\expandafter\def\csname R@maes/trans/share\endcsname{0.9}
\expandafter\def\csname R@maes/trans/t/336\endcsname{1.55}
\expandafter\def\csname R@maes/trans/t/6\endcsname{1.70}
\expandafter\def\csname R@maes/v5/0\endcsname{0.978}
\expandafter\def\csname R@maes/v5/0/n\endcsname{1}
\expandafter\def\csname R@maes/v5/18\endcsname{0.881}
\expandafter\def\csname R@maes/v5/18/ep/max\endcsname{13}
\expandafter\def\csname R@maes/v5/18/ep/min\endcsname{11}
\expandafter\def\csname R@maes/v5/18/n\endcsname{3}
\expandafter\def\csname R@maes/v5/18/sd\endcsname{0.000}
\expandafter\def\csname R@maes/v5/192\endcsname{0.878}
\expandafter\def\csname R@maes/v5/192/ep/max\endcsname{12}
\expandafter\def\csname R@maes/v5/192/ep/min\endcsname{9}
\expandafter\def\csname R@maes/v5/192/n\endcsname{3}
\expandafter\def\csname R@maes/v5/192/sd\endcsname{0.000}
\expandafter\def\csname R@maes/v5/336\endcsname{0.878}
\expandafter\def\csname R@maes/v5/336/ep/max\endcsname{17}
\expandafter\def\csname R@maes/v5/336/ep/min\endcsname{15}
\expandafter\def\csname R@maes/v5/336/n\endcsname{3}
\expandafter\def\csname R@maes/v5/336/sd\endcsname{0.000}
\expandafter\def\csname R@maes/v5/48\endcsname{0.879}
\expandafter\def\csname R@maes/v5/48/ep/max\endcsname{12}
\expandafter\def\csname R@maes/v5/48/ep/min\endcsname{10}
\expandafter\def\csname R@maes/v5/48/n\endcsname{3}
\expandafter\def\csname R@maes/v5/48/sd\endcsname{0.000}
\expandafter\def\csname R@maes/v5/6\endcsname{0.887}
\expandafter\def\csname R@maes/v5/6/ep/max\endcsname{14}
\expandafter\def\csname R@maes/v5/6/ep/min\endcsname{12}
\expandafter\def\csname R@maes/v5/6/n\endcsname{3}
\expandafter\def\csname R@maes/v5/6/sd\endcsname{0.000}
\expandafter\def\csname R@maes/v5/96\endcsname{0.879}
\expandafter\def\csname R@maes/v5/96/ep/max\endcsname{12}
\expandafter\def\csname R@maes/v5/96/ep/min\endcsname{8}
\expandafter\def\csname R@maes/v5/96/n\endcsname{3}
\expandafter\def\csname R@maes/v5/96/sd\endcsname{0.000}
\expandafter\def\csname R@maes/v5/ep/max\endcsname{17}
\expandafter\def\csname R@maes/v5/maxsd\endcsname{0.000}
\expandafter\def\csname R@maes/win/test\endcsname{1113}
\expandafter\def\csname R@maes/win/train\endcsname{9072}
\expandafter\def\csname R@maes/window\endcsname{480}
\expandafter\def\csname R@maes48/boot/t/6-336\endcsname{0.299}
\expandafter\def\csname R@maes48/boot/t/6-336/hi\endcsname{0.321}
\expandafter\def\csname R@maes48/boot/t/6-336/lo\endcsname{0.279}
\expandafter\def\csname R@maes48/boot/t/96-336\endcsname{0.047}
\expandafter\def\csname R@maes48/boot/t/96-336/hi\endcsname{0.054}
\expandafter\def\csname R@maes48/boot/t/96-336/lo\endcsname{0.041}
\expandafter\def\csname R@maes48/copybase/backoff/gain\endcsname{11}
\expandafter\def\csname R@maes48/reached/t/96\endcsname{84}
\expandafter\def\csname R@maes48/redshare/t/none\endcsname{98.2}
\expandafter\def\csname R@maes48/share/t/repeat\endcsname{0.82}
\expandafter\def\csname R@maes48/tok/336\endcsname{2.830}
\expandafter\def\csname R@maes48/tok/6\endcsname{3.129}
\expandafter\def\csname R@maes48/tok/drop\endcsname{10}
\expandafter\def\csname R@maesd32/ae/acc\endcsname{90.223}
\expandafter\def\csname R@music/abl/t/repl/18\endcsname{2.552}
\expandafter\def\csname R@music/abl/t/repl/18/none\endcsname{2.564}
\expandafter\def\csname R@music/abl/t/repl/18/repeat\endcsname{2.450}
\expandafter\def\csname R@music/abl/t/repl/192\endcsname{2.098}
\expandafter\def\csname R@music/abl/t/repl/192/none\endcsname{2.157}
\expandafter\def\csname R@music/abl/t/repl/192/repeat\endcsname{1.598}
\expandafter\def\csname R@music/abl/t/repl/48\endcsname{2.301}
\expandafter\def\csname R@music/abl/t/repl/48/none\endcsname{2.332}
\expandafter\def\csname R@music/abl/t/repl/48/repeat\endcsname{2.040}
\expandafter\def\csname R@music/abl/t/repl/6\endcsname{3.118}
\expandafter\def\csname R@music/abl/t/repl/6/none\endcsname{3.107}
\expandafter\def\csname R@music/abl/t/repl/6/repeat\endcsname{3.215}
\expandafter\def\csname R@music/abl/t/repl/96\endcsname{2.173}
\expandafter\def\csname R@music/abl/t/repl/96/none\endcsname{2.220}
\expandafter\def\csname R@music/abl/t/repl/96/repeat\endcsname{1.775}
\expandafter\def\csname R@music/abl/t/sweep/18\endcsname{2.366}
\expandafter\def\csname R@music/abl/t/sweep/192\endcsname{2.050}
\expandafter\def\csname R@music/abl/t/sweep/336\endcsname{2.067}
\expandafter\def\csname R@music/abl/t/sweep/48\endcsname{2.159}
\expandafter\def\csname R@music/abl/t/sweep/6\endcsname{2.512}
\expandafter\def\csname R@music/abl/t/sweep/96\endcsname{2.080}
\expandafter\def\csname R@music/abl/t/trunc/18\endcsname{2.339}
\expandafter\def\csname R@music/abl/t/trunc/18/none\endcsname{2.361}
\expandafter\def\csname R@music/abl/t/trunc/18/repeat\endcsname{2.155}
\expandafter\def\csname R@music/abl/t/trunc/192\endcsname{2.077}
\expandafter\def\csname R@music/abl/t/trunc/192/none\endcsname{2.139}
\expandafter\def\csname R@music/abl/t/trunc/192/repeat\endcsname{1.550}
\expandafter\def\csname R@music/abl/t/trunc/336\endcsname{2.067}
\expandafter\def\csname R@music/abl/t/trunc/336/none\endcsname{2.134}
\expandafter\def\csname R@music/abl/t/trunc/336/repeat\endcsname{1.498}
\expandafter\def\csname R@music/abl/t/trunc/48\endcsname{2.196}
\expandafter\def\csname R@music/abl/t/trunc/48/none\endcsname{2.230}
\expandafter\def\csname R@music/abl/t/trunc/48/repeat\endcsname{1.907}
\expandafter\def\csname R@music/abl/t/trunc/6\endcsname{2.730}
\expandafter\def\csname R@music/abl/t/trunc/6/none\endcsname{2.724}
\expandafter\def\csname R@music/abl/t/trunc/6/repeat\endcsname{2.783}
\expandafter\def\csname R@music/abl/t/trunc/96\endcsname{2.115}
\expandafter\def\csname R@music/abl/t/trunc/96/none\endcsname{2.165}
\expandafter\def\csname R@music/abl/t/trunc/96/repeat\endcsname{1.685}
\expandafter\def\csname R@music/abl/targets\endcsname{31{,}392}
\expandafter\def\csname R@music/boot/t/18-48\endcsname{0.207}
\expandafter\def\csname R@music/boot/t/18-48/hi\endcsname{0.251}
\expandafter\def\csname R@music/boot/t/18-48/lo\endcsname{0.166}
\expandafter\def\csname R@music/boot/t/18-6\endcsname{-0.146}
\expandafter\def\csname R@music/boot/t/18-6/hi\endcsname{-0.117}
\expandafter\def\csname R@music/boot/t/18-6/lo\endcsname{-0.177}
\expandafter\def\csname R@music/boot/t/192-336\endcsname{-0.017}
\expandafter\def\csname R@music/boot/t/192-336/hi\endcsname{-0.004}
\expandafter\def\csname R@music/boot/t/192-336/lo\endcsname{-0.029}
\expandafter\def\csname R@music/boot/t/192-96\endcsname{-0.029}
\expandafter\def\csname R@music/boot/t/192-96/hi\endcsname{-0.012}
\expandafter\def\csname R@music/boot/t/192-96/lo\endcsname{-0.049}
\expandafter\def\csname R@music/boot/t/336-192\endcsname{0.017}
\expandafter\def\csname R@music/boot/t/336-192/hi\endcsname{0.029}
\expandafter\def\csname R@music/boot/t/336-192/lo\endcsname{0.004}
\expandafter\def\csname R@music/boot/t/336-48\endcsname{-0.092}
\expandafter\def\csname R@music/boot/t/336-48/hi\endcsname{-0.051}
\expandafter\def\csname R@music/boot/t/336-48/lo\endcsname{-0.136}
\expandafter\def\csname R@music/boot/t/336-6\endcsname{-0.445}
\expandafter\def\csname R@music/boot/t/336-6/hi\endcsname{-0.369}
\expandafter\def\csname R@music/boot/t/336-6/lo\endcsname{-0.524}
\expandafter\def\csname R@music/boot/t/336-96\endcsname{-0.013}
\expandafter\def\csname R@music/boot/t/336-96/hi\endcsname{0.011}
\expandafter\def\csname R@music/boot/t/336-96/lo\endcsname{-0.039}
\expandafter\def\csname R@music/boot/t/48-18\endcsname{-0.207}
\expandafter\def\csname R@music/boot/t/48-18/hi\endcsname{-0.166}
\expandafter\def\csname R@music/boot/t/48-18/lo\endcsname{-0.251}
\expandafter\def\csname R@music/boot/t/48-336\endcsname{0.092}
\expandafter\def\csname R@music/boot/t/48-336/hi\endcsname{0.136}
\expandafter\def\csname R@music/boot/t/48-336/lo\endcsname{0.051}
\expandafter\def\csname R@music/boot/t/48-96\endcsname{0.080}
\expandafter\def\csname R@music/boot/t/48-96/hi\endcsname{0.106}
\expandafter\def\csname R@music/boot/t/48-96/lo\endcsname{0.054}
\expandafter\def\csname R@music/boot/t/6-18\endcsname{0.146}
\expandafter\def\csname R@music/boot/t/6-18/hi\endcsname{0.177}
\expandafter\def\csname R@music/boot/t/6-18/lo\endcsname{0.117}
\expandafter\def\csname R@music/boot/t/6-336\endcsname{0.445}
\expandafter\def\csname R@music/boot/t/6-336/hi\endcsname{0.524}
\expandafter\def\csname R@music/boot/t/6-336/lo\endcsname{0.369}
\expandafter\def\csname R@music/boot/t/96-192\endcsname{0.029}
\expandafter\def\csname R@music/boot/t/96-192/hi\endcsname{0.049}
\expandafter\def\csname R@music/boot/t/96-192/lo\endcsname{0.012}
\expandafter\def\csname R@music/boot/t/96-336\endcsname{0.013}
\expandafter\def\csname R@music/boot/t/96-336/hi\endcsname{0.039}
\expandafter\def\csname R@music/boot/t/96-336/lo\endcsname{-0.011}
\expandafter\def\csname R@music/boot/t/96-48\endcsname{-0.080}
\expandafter\def\csname R@music/boot/t/96-48/hi\endcsname{-0.054}
\expandafter\def\csname R@music/boot/t/96-48/lo\endcsname{-0.106}
\expandafter\def\csname R@music/clamp/rep16/clamped\endcsname{10.49}
\expandafter\def\csname R@music/clamp/rep16/full\endcsname{10.47}
\expandafter\def\csname R@music/clamp/rep8/clamped\endcsname{17.69}
\expandafter\def\csname R@music/clamp/rep8/full\endcsname{17.66}
\expandafter\def\csname R@music/clamped\endcsname{2.2}
\expandafter\def\csname R@music/copy/t/1-32\endcsname{90}
\expandafter\def\csname R@music/copy/t/177-320\endcsname{98}
\expandafter\def\csname R@music/copy/t/33-80\endcsname{95}
\expandafter\def\csname R@music/copy/t/81-176\endcsname{96}
\expandafter\def\csname R@music/copy/t/all\endcsname{94}
\expandafter\def\csname R@music/copybase/16\endcsname{2.304}
\expandafter\def\csname R@music/copybase/16/gain\endcsname{47}
\expandafter\def\csname R@music/copybase/16/matched\endcsname{10}
\expandafter\def\csname R@music/copybase/backoff\endcsname{2.191}
\expandafter\def\csname R@music/copybase/backoff/gain\endcsname{72}
\expandafter\def\csname R@music/copybase/backoff/matched\endcsname{18}
\expandafter\def\csname R@music/copybase/base\endcsname{2.512}
\expandafter\def\csname R@music/copybase/m/bits_T336\endcsname{1.60}
\expandafter\def\csname R@music/copybase/m/bits_T6\endcsname{2.62}
\expandafter\def\csname R@music/copybase/m/bits_copy\endcsname{0.88}
\expandafter\def\csname R@music/copybase/m/copy\endcsname{72}
\expandafter\def\csname R@music/copybase/m/t336\endcsname{42}
\expandafter\def\csname R@music/groups\endcsname{297}
\expandafter\def\csname R@music/h32/copy\endcsname{96}
\expandafter\def\csname R@music/h32/redshare/t\endcsname{10}
\expandafter\def\csname R@music/h32/share\endcsname{5}
\expandafter\def\csname R@music/h8/copy\endcsname{89}
\expandafter\def\csname R@music/h8/redshare/t\endcsname{41}
\expandafter\def\csname R@music/h8/share\endcsname{18}
\expandafter\def\csname R@music/inview/18\endcsname{0.0}
\expandafter\def\csname R@music/inview/192\endcsname{8.3}
\expandafter\def\csname R@music/inview/336\endcsname{10.5}
\expandafter\def\csname R@music/inview/48\endcsname{3.1}
\expandafter\def\csname R@music/inview/6\endcsname{0.0}
\expandafter\def\csname R@music/inview/96\endcsname{5.9}
\expandafter\def\csname R@music/lag/t/18/1-32\endcsname{2.52}
\expandafter\def\csname R@music/lag/t/18/177-320\endcsname{2.36}
\expandafter\def\csname R@music/lag/t/18/33-80\endcsname{2.21}
\expandafter\def\csname R@music/lag/t/18/81-176\endcsname{2.39}
\expandafter\def\csname R@music/lag/t/18/held\endcsname{1.24}
\expandafter\def\csname R@music/lag/t/18/none\endcsname{2.41}
\expandafter\def\csname R@music/lag/t/192/1-32\endcsname{1.48}
\expandafter\def\csname R@music/lag/t/192/177-320\endcsname{1.99}
\expandafter\def\csname R@music/lag/t/192/33-80\endcsname{1.36}
\expandafter\def\csname R@music/lag/t/192/81-176\endcsname{1.60}
\expandafter\def\csname R@music/lag/t/192/held\endcsname{1.12}
\expandafter\def\csname R@music/lag/t/192/none\endcsname{2.14}
\expandafter\def\csname R@music/lag/t/336/1-32\endcsname{1.44}
\expandafter\def\csname R@music/lag/t/336/177-320\endcsname{1.62}
\expandafter\def\csname R@music/lag/t/336/33-80\endcsname{1.35}
\expandafter\def\csname R@music/lag/t/336/81-176\endcsname{1.64}
\expandafter\def\csname R@music/lag/t/336/held\endcsname{1.13}
\expandafter\def\csname R@music/lag/t/336/none\endcsname{2.17}
\expandafter\def\csname R@music/lag/t/48/1-32\endcsname{1.87}
\expandafter\def\csname R@music/lag/t/48/177-320\endcsname{2.13}
\expandafter\def\csname R@music/lag/t/48/33-80\endcsname{2.01}
\expandafter\def\csname R@music/lag/t/48/81-176\endcsname{2.15}
\expandafter\def\csname R@music/lag/t/48/held\endcsname{1.19}
\expandafter\def\csname R@music/lag/t/48/none\endcsname{2.21}
\expandafter\def\csname R@music/lag/t/6/1-32\endcsname{2.83}
\expandafter\def\csname R@music/lag/t/6/177-320\endcsname{2.47}
\expandafter\def\csname R@music/lag/t/6/33-80\endcsname{2.35}
\expandafter\def\csname R@music/lag/t/6/81-176\endcsname{2.53}
\expandafter\def\csname R@music/lag/t/6/held\endcsname{1.23}
\expandafter\def\csname R@music/lag/t/6/none\endcsname{2.55}
\expandafter\def\csname R@music/lag/t/96/1-32\endcsname{1.53}
\expandafter\def\csname R@music/lag/t/96/177-320\endcsname{2.06}
\expandafter\def\csname R@music/lag/t/96/33-80\endcsname{1.43}
\expandafter\def\csname R@music/lag/t/96/81-176\endcsname{2.09}
\expandafter\def\csname R@music/lag/t/96/held\endcsname{1.12}
\expandafter\def\csname R@music/lag/t/96/none\endcsname{2.16}
\expandafter\def\csname R@music/leak/test/verbatim\endcsname{0.0}
\expandafter\def\csname R@music/lenratio\endcsname{1.97}
\expandafter\def\csname R@music/longep/max\endcsname{25}
\expandafter\def\csname R@music/longep/min\endcsname{20}
\expandafter\def\csname R@music/moved\endcsname{0}
\expandafter\def\csname R@music/pieces/all\endcsname{323}
\expandafter\def\csname R@music/pieces/test\endcsname{48}
\expandafter\def\csname R@music/pieces/testwin\endcsname{43}
\expandafter\def\csname R@music/pieces/train\endcsname{221}
\expandafter\def\csname R@music/pieces/val\endcsname{54}
\expandafter\def\csname R@music/pitchlo\endcsname{47}
\expandafter\def\csname R@music/reached/t/18\endcsname{33}
\expandafter\def\csname R@music/reached/t/192\endcsname{104}
\expandafter\def\csname R@music/reached/t/336\endcsname{100}
\expandafter\def\csname R@music/reached/t/48\endcsname{79}
\expandafter\def\csname R@music/reached/t/6\endcsname{0}
\expandafter\def\csname R@music/reached/t/96\endcsname{97}
\expandafter\def\csname R@music/redshare/t/none\endcsname{74}
\expandafter\def\csname R@music/redshare/t/repeat\endcsname{25}
\expandafter\def\csname R@music/rest\endcsname{5.2}
\expandafter\def\csname R@music/share/t/1-32\endcsname{3.1}
\expandafter\def\csname R@music/share/t/177-320\endcsname{2.2}
\expandafter\def\csname R@music/share/t/33-80\endcsname{2.8}
\expandafter\def\csname R@music/share/t/81-176\endcsname{2.4}
\expandafter\def\csname R@music/share/t/held\endcsname{3.1}
\expandafter\def\csname R@music/share/t/none\endcsname{86.4}
\expandafter\def\csname R@music/share/t/repeat\endcsname{10}
\expandafter\def\csname R@music/targets\endcsname{144}
\expandafter\def\csname R@music/tok/0\endcsname{5.295}
\expandafter\def\csname R@music/tok/0/n\endcsname{1}
\expandafter\def\csname R@music/tok/18\endcsname{2.366}
\expandafter\def\csname R@music/tok/18/ep/max\endcsname{23}
\expandafter\def\csname R@music/tok/18/ep/min\endcsname{20}
\expandafter\def\csname R@music/tok/18/n\endcsname{3}
\expandafter\def\csname R@music/tok/18/sd\endcsname{0.003}
\expandafter\def\csname R@music/tok/192\endcsname{2.050}
\expandafter\def\csname R@music/tok/192/ep/max\endcsname{25}
\expandafter\def\csname R@music/tok/192/ep/min\endcsname{21}
\expandafter\def\csname R@music/tok/192/n\endcsname{3}
\expandafter\def\csname R@music/tok/192/sd\endcsname{0.009}
\expandafter\def\csname R@music/tok/336\endcsname{2.067}
\expandafter\def\csname R@music/tok/336/ep/max\endcsname{24}
\expandafter\def\csname R@music/tok/336/ep/min\endcsname{20}
\expandafter\def\csname R@music/tok/336/n\endcsname{3}
\expandafter\def\csname R@music/tok/336/sd\endcsname{0.004}
\expandafter\def\csname R@music/tok/48\endcsname{2.159}
\expandafter\def\csname R@music/tok/48/ep/max\endcsname{20}
\expandafter\def\csname R@music/tok/48/ep/min\endcsname{17}
\expandafter\def\csname R@music/tok/48/n\endcsname{3}
\expandafter\def\csname R@music/tok/48/sd\endcsname{0.004}
\expandafter\def\csname R@music/tok/6\endcsname{2.512}
\expandafter\def\csname R@music/tok/6/ep/max\endcsname{23}
\expandafter\def\csname R@music/tok/6/ep/min\endcsname{18}
\expandafter\def\csname R@music/tok/6/n\endcsname{3}
\expandafter\def\csname R@music/tok/6/sd\endcsname{0.066}
\expandafter\def\csname R@music/tok/96\endcsname{2.080}
\expandafter\def\csname R@music/tok/96/ep/max\endcsname{22}
\expandafter\def\csname R@music/tok/96/ep/min\endcsname{19}
\expandafter\def\csname R@music/tok/96/n\endcsname{3}
\expandafter\def\csname R@music/tok/96/sd\endcsname{0.003}
\expandafter\def\csname R@music/tok/drop\endcsname{18}
\expandafter\def\csname R@music/tok/ep/max\endcsname{25}
\expandafter\def\csname R@music/tok/maxsd\endcsname{0.066}
\expandafter\def\csname R@music/tokens/test\endcsname{115{,}563}
\expandafter\def\csname R@music/tokens/train\endcsname{576{,}974}
\expandafter\def\csname R@music/tokens/val\endcsname{140{,}713}
\expandafter\def\csname R@music/trans/copy\endcsname{90}
\expandafter\def\csname R@music/trans/other/336\endcsname{2.21}
\expandafter\def\csname R@music/trans/other/6\endcsname{2.59}
\expandafter\def\csname R@music/trans/share\endcsname{8.0}
\expandafter\def\csname R@music/trans/t/336\endcsname{1.76}
\expandafter\def\csname R@music/trans/t/6\endcsname{2.15}
\expandafter\def\csname R@music/win/test\endcsname{218}
\expandafter\def\csname R@music/win/train\endcsname{1091}
\expandafter\def\csname R@music/window\endcsname{480}
\expandafter\def\csname R@nott/abl/l/repl/18\endcsname{0.956}
\expandafter\def\csname R@nott/abl/l/repl/18/none\endcsname{0.959}
\expandafter\def\csname R@nott/abl/l/repl/18/repeat\endcsname{0.954}
\expandafter\def\csname R@nott/abl/l/repl/192\endcsname{0.571}
\expandafter\def\csname R@nott/abl/l/repl/192/none\endcsname{0.793}
\expandafter\def\csname R@nott/abl/l/repl/192/repeat\endcsname{0.483}
\expandafter\def\csname R@nott/abl/l/repl/48\endcsname{0.935}
\expandafter\def\csname R@nott/abl/l/repl/48/none\endcsname{0.942}
\expandafter\def\csname R@nott/abl/l/repl/48/repeat\endcsname{0.932}
\expandafter\def\csname R@nott/abl/l/repl/6\endcsname{0.994}
\expandafter\def\csname R@nott/abl/l/repl/6/none\endcsname{1.001}
\expandafter\def\csname R@nott/abl/l/repl/6/repeat\endcsname{0.991}
\expandafter\def\csname R@nott/abl/l/repl/96\endcsname{0.837}
\expandafter\def\csname R@nott/abl/l/repl/96/none\endcsname{0.890}
\expandafter\def\csname R@nott/abl/l/repl/96/repeat\endcsname{0.815}
\expandafter\def\csname R@nott/abl/l/trunc/18\endcsname{1.278}
\expandafter\def\csname R@nott/abl/l/trunc/18/none\endcsname{1.274}
\expandafter\def\csname R@nott/abl/l/trunc/18/repeat\endcsname{1.280}
\expandafter\def\csname R@nott/abl/l/trunc/192\endcsname{0.562}
\expandafter\def\csname R@nott/abl/l/trunc/192/none\endcsname{0.801}
\expandafter\def\csname R@nott/abl/l/trunc/192/repeat\endcsname{0.467}
\expandafter\def\csname R@nott/abl/l/trunc/336\endcsname{0.465}
\expandafter\def\csname R@nott/abl/l/trunc/336/none\endcsname{0.762}
\expandafter\def\csname R@nott/abl/l/trunc/336/repeat\endcsname{0.346}
\expandafter\def\csname R@nott/abl/l/trunc/48\endcsname{0.992}
\expandafter\def\csname R@nott/abl/l/trunc/48/none\endcsname{0.997}
\expandafter\def\csname R@nott/abl/l/trunc/48/repeat\endcsname{0.990}
\expandafter\def\csname R@nott/abl/l/trunc/6\endcsname{1.710}
\expandafter\def\csname R@nott/abl/l/trunc/6/none\endcsname{1.680}
\expandafter\def\csname R@nott/abl/l/trunc/6/repeat\endcsname{1.722}
\expandafter\def\csname R@nott/abl/l/trunc/96\endcsname{0.833}
\expandafter\def\csname R@nott/abl/l/trunc/96/none\endcsname{0.895}
\expandafter\def\csname R@nott/abl/l/trunc/96/repeat\endcsname{0.808}
\expandafter\def\csname R@nott/abl/t/repl/18\endcsname{1.557}
\expandafter\def\csname R@nott/abl/t/repl/18/none\endcsname{1.536}
\expandafter\def\csname R@nott/abl/t/repl/18/repeat\endcsname{1.565}
\expandafter\def\csname R@nott/abl/t/repl/192\endcsname{0.591}
\expandafter\def\csname R@nott/abl/t/repl/192/none\endcsname{1.015}
\expandafter\def\csname R@nott/abl/t/repl/192/repeat\endcsname{0.418}
\expandafter\def\csname R@nott/abl/t/repl/48\endcsname{1.417}
\expandafter\def\csname R@nott/abl/t/repl/48/none\endcsname{1.417}
\expandafter\def\csname R@nott/abl/t/repl/48/repeat\endcsname{1.417}
\expandafter\def\csname R@nott/abl/t/repl/6\endcsname{1.692}
\expandafter\def\csname R@nott/abl/t/repl/6/none\endcsname{1.673}
\expandafter\def\csname R@nott/abl/t/repl/6/repeat\endcsname{1.700}
\expandafter\def\csname R@nott/abl/t/repl/96\endcsname{1.078}
\expandafter\def\csname R@nott/abl/t/repl/96/none\endcsname{1.223}
\expandafter\def\csname R@nott/abl/t/repl/96/repeat\endcsname{1.019}
\expandafter\def\csname R@nott/abl/t/sweep/18\endcsname{1.440}
\expandafter\def\csname R@nott/abl/t/sweep/192\endcsname{0.567}
\expandafter\def\csname R@nott/abl/t/sweep/336\endcsname{0.405}
\expandafter\def\csname R@nott/abl/t/sweep/48\endcsname{1.529}
\expandafter\def\csname R@nott/abl/t/sweep/6\endcsname{1.391}
\expandafter\def\csname R@nott/abl/t/sweep/96\endcsname{1.274}
\expandafter\def\csname R@nott/abl/t/trunc/18\endcsname{1.543}
\expandafter\def\csname R@nott/abl/t/trunc/18/none\endcsname{1.528}
\expandafter\def\csname R@nott/abl/t/trunc/18/repeat\endcsname{1.550}
\expandafter\def\csname R@nott/abl/t/trunc/192\endcsname{0.576}
\expandafter\def\csname R@nott/abl/t/trunc/192/none\endcsname{0.997}
\expandafter\def\csname R@nott/abl/t/trunc/192/repeat\endcsname{0.404}
\expandafter\def\csname R@nott/abl/t/trunc/336\endcsname{0.405}
\expandafter\def\csname R@nott/abl/t/trunc/336/none\endcsname{0.933}
\expandafter\def\csname R@nott/abl/t/trunc/336/repeat\endcsname{0.190}
\expandafter\def\csname R@nott/abl/t/trunc/48\endcsname{1.355}
\expandafter\def\csname R@nott/abl/t/trunc/48/none\endcsname{1.345}
\expandafter\def\csname R@nott/abl/t/trunc/48/repeat\endcsname{1.359}
\expandafter\def\csname R@nott/abl/t/trunc/6\endcsname{1.831}
\expandafter\def\csname R@nott/abl/t/trunc/6/none\endcsname{1.791}
\expandafter\def\csname R@nott/abl/t/trunc/6/repeat\endcsname{1.847}
\expandafter\def\csname R@nott/abl/t/trunc/96\endcsname{1.008}
\expandafter\def\csname R@nott/abl/t/trunc/96/none\endcsname{1.146}
\expandafter\def\csname R@nott/abl/t/trunc/96/repeat\endcsname{0.951}
\expandafter\def\csname R@nott/abl/targets\endcsname{31{,}680}
\expandafter\def\csname R@nott/ae/acc\endcsname{99.923}
\expandafter\def\csname R@nott/align/192/aligned\endcsname{0.31}
\expandafter\def\csname R@nott/align/192/misaligned\endcsname{0.32}
\expandafter\def\csname R@nott/align/192/share\endcsname{26}
\expandafter\def\csname R@nott/align/336/aligned\endcsname{0.20}
\expandafter\def\csname R@nott/align/336/misaligned\endcsname{0.34}
\expandafter\def\csname R@nott/align/336/share\endcsname{34}
\expandafter\def\csname R@nott/align/96/aligned\endcsname{0.73}
\expandafter\def\csname R@nott/align/96/misaligned\endcsname{0.55}
\expandafter\def\csname R@nott/align/96/share\endcsname{17}
\expandafter\def\csname R@nott/aligned/1-32\endcsname{24}
\expandafter\def\csname R@nott/aligned/177-320\endcsname{54}
\expandafter\def\csname R@nott/aligned/33-80\endcsname{22}
\expandafter\def\csname R@nott/aligned/81-176\endcsname{31}
\expandafter\def\csname R@nott/aligned/all\endcsname{34}
\expandafter\def\csname R@nott/boot/l/18-48\endcsname{0.007}
\expandafter\def\csname R@nott/boot/l/18-48/hi\endcsname{0.011}
\expandafter\def\csname R@nott/boot/l/18-48/lo\endcsname{0.004}
\expandafter\def\csname R@nott/boot/l/18-6\endcsname{-0.015}
\expandafter\def\csname R@nott/boot/l/18-6/hi\endcsname{-0.011}
\expandafter\def\csname R@nott/boot/l/18-6/lo\endcsname{-0.018}
\expandafter\def\csname R@nott/boot/l/192-336\endcsname{0.105}
\expandafter\def\csname R@nott/boot/l/192-336/hi\endcsname{0.148}
\expandafter\def\csname R@nott/boot/l/192-336/lo\endcsname{0.068}
\expandafter\def\csname R@nott/boot/l/192-96\endcsname{-0.205}
\expandafter\def\csname R@nott/boot/l/192-96/hi\endcsname{-0.160}
\expandafter\def\csname R@nott/boot/l/192-96/lo\endcsname{-0.247}
\expandafter\def\csname R@nott/boot/l/336-192\endcsname{-0.105}
\expandafter\def\csname R@nott/boot/l/336-192/hi\endcsname{-0.068}
\expandafter\def\csname R@nott/boot/l/336-192/lo\endcsname{-0.148}
\expandafter\def\csname R@nott/boot/l/336-48\endcsname{-0.369}
\expandafter\def\csname R@nott/boot/l/336-48/hi\endcsname{-0.339}
\expandafter\def\csname R@nott/boot/l/336-48/lo\endcsname{-0.397}
\expandafter\def\csname R@nott/boot/l/336-6\endcsname{-0.392}
\expandafter\def\csname R@nott/boot/l/336-6/hi\endcsname{-0.362}
\expandafter\def\csname R@nott/boot/l/336-6/lo\endcsname{-0.419}
\expandafter\def\csname R@nott/boot/l/336-96\endcsname{-0.310}
\expandafter\def\csname R@nott/boot/l/336-96/hi\endcsname{-0.283}
\expandafter\def\csname R@nott/boot/l/336-96/lo\endcsname{-0.335}
\expandafter\def\csname R@nott/boot/l/48-18\endcsname{-0.007}
\expandafter\def\csname R@nott/boot/l/48-18/hi\endcsname{-0.004}
\expandafter\def\csname R@nott/boot/l/48-18/lo\endcsname{-0.011}
\expandafter\def\csname R@nott/boot/l/48-336\endcsname{0.369}
\expandafter\def\csname R@nott/boot/l/48-336/hi\endcsname{0.397}
\expandafter\def\csname R@nott/boot/l/48-336/lo\endcsname{0.339}
\expandafter\def\csname R@nott/boot/l/48-96\endcsname{0.059}
\expandafter\def\csname R@nott/boot/l/48-96/hi\endcsname{0.080}
\expandafter\def\csname R@nott/boot/l/48-96/lo\endcsname{0.040}
\expandafter\def\csname R@nott/boot/l/6-18\endcsname{0.015}
\expandafter\def\csname R@nott/boot/l/6-18/hi\endcsname{0.018}
\expandafter\def\csname R@nott/boot/l/6-18/lo\endcsname{0.011}
\expandafter\def\csname R@nott/boot/l/6-336\endcsname{0.392}
\expandafter\def\csname R@nott/boot/l/6-336/hi\endcsname{0.419}
\expandafter\def\csname R@nott/boot/l/6-336/lo\endcsname{0.362}
\expandafter\def\csname R@nott/boot/l/96-192\endcsname{0.205}
\expandafter\def\csname R@nott/boot/l/96-192/hi\endcsname{0.247}
\expandafter\def\csname R@nott/boot/l/96-192/lo\endcsname{0.160}
\expandafter\def\csname R@nott/boot/l/96-336\endcsname{0.310}
\expandafter\def\csname R@nott/boot/l/96-336/hi\endcsname{0.335}
\expandafter\def\csname R@nott/boot/l/96-336/lo\endcsname{0.283}
\expandafter\def\csname R@nott/boot/l/96-48\endcsname{-0.059}
\expandafter\def\csname R@nott/boot/l/96-48/hi\endcsname{-0.040}
\expandafter\def\csname R@nott/boot/l/96-48/lo\endcsname{-0.080}
\expandafter\def\csname R@nott/boot/t/18-48\endcsname{-0.089}
\expandafter\def\csname R@nott/boot/t/18-48/hi\endcsname{-0.067}
\expandafter\def\csname R@nott/boot/t/18-48/lo\endcsname{-0.111}
\expandafter\def\csname R@nott/boot/t/18-6\endcsname{0.049}
\expandafter\def\csname R@nott/boot/t/18-6/hi\endcsname{0.069}
\expandafter\def\csname R@nott/boot/t/18-6/lo\endcsname{0.028}
\expandafter\def\csname R@nott/boot/t/192-336\endcsname{0.162}
\expandafter\def\csname R@nott/boot/t/192-336/hi\endcsname{0.223}
\expandafter\def\csname R@nott/boot/t/192-336/lo\endcsname{0.101}
\expandafter\def\csname R@nott/boot/t/192-96\endcsname{-0.707}
\expandafter\def\csname R@nott/boot/t/192-96/hi\endcsname{-0.633}
\expandafter\def\csname R@nott/boot/t/192-96/lo\endcsname{-0.784}
\expandafter\def\csname R@nott/boot/t/336-192\endcsname{-0.162}
\expandafter\def\csname R@nott/boot/t/336-192/hi\endcsname{-0.101}
\expandafter\def\csname R@nott/boot/t/336-192/lo\endcsname{-0.223}
\expandafter\def\csname R@nott/boot/t/336-48\endcsname{-1.124}
\expandafter\def\csname R@nott/boot/t/336-48/hi\endcsname{-1.056}
\expandafter\def\csname R@nott/boot/t/336-48/lo\endcsname{-1.195}
\expandafter\def\csname R@nott/boot/t/336-6\endcsname{-0.986}
\expandafter\def\csname R@nott/boot/t/336-6/hi\endcsname{-0.925}
\expandafter\def\csname R@nott/boot/t/336-6/lo\endcsname{-1.051}
\expandafter\def\csname R@nott/boot/t/336-96\endcsname{-0.869}
\expandafter\def\csname R@nott/boot/t/336-96/hi\endcsname{-0.817}
\expandafter\def\csname R@nott/boot/t/336-96/lo\endcsname{-0.924}
\expandafter\def\csname R@nott/boot/t/48-18\endcsname{0.089}
\expandafter\def\csname R@nott/boot/t/48-18/hi\endcsname{0.111}
\expandafter\def\csname R@nott/boot/t/48-18/lo\endcsname{0.067}
\expandafter\def\csname R@nott/boot/t/48-336\endcsname{1.124}
\expandafter\def\csname R@nott/boot/t/48-336/hi\endcsname{1.195}
\expandafter\def\csname R@nott/boot/t/48-336/lo\endcsname{1.056}
\expandafter\def\csname R@nott/boot/t/48-96\endcsname{0.255}
\expandafter\def\csname R@nott/boot/t/48-96/hi\endcsname{0.304}
\expandafter\def\csname R@nott/boot/t/48-96/lo\endcsname{0.205}
\expandafter\def\csname R@nott/boot/t/6-18\endcsname{-0.049}
\expandafter\def\csname R@nott/boot/t/6-18/hi\endcsname{-0.028}
\expandafter\def\csname R@nott/boot/t/6-18/lo\endcsname{-0.069}
\expandafter\def\csname R@nott/boot/t/6-336\endcsname{0.986}
\expandafter\def\csname R@nott/boot/t/6-336/hi\endcsname{1.051}
\expandafter\def\csname R@nott/boot/t/6-336/lo\endcsname{0.925}
\expandafter\def\csname R@nott/boot/t/96-192\endcsname{0.707}
\expandafter\def\csname R@nott/boot/t/96-192/hi\endcsname{0.784}
\expandafter\def\csname R@nott/boot/t/96-192/lo\endcsname{0.633}
\expandafter\def\csname R@nott/boot/t/96-336\endcsname{0.869}
\expandafter\def\csname R@nott/boot/t/96-336/hi\endcsname{0.924}
\expandafter\def\csname R@nott/boot/t/96-336/lo\endcsname{0.817}
\expandafter\def\csname R@nott/boot/t/96-48\endcsname{-0.255}
\expandafter\def\csname R@nott/boot/t/96-48/hi\endcsname{-0.205}
\expandafter\def\csname R@nott/boot/t/96-48/lo\endcsname{-0.304}
\expandafter\def\csname R@nott/clamped\endcsname{0.0}
\expandafter\def\csname R@nott/copy/s/1-32\endcsname{35}
\expandafter\def\csname R@nott/copy/s/177-320\endcsname{94}
\expandafter\def\csname R@nott/copy/s/33-80\endcsname{70}
\expandafter\def\csname R@nott/copy/s/81-176\endcsname{92}
\expandafter\def\csname R@nott/copy/s/all\endcsname{86}
\expandafter\def\csname R@nott/copy/t/1-32\endcsname{82}
\expandafter\def\csname R@nott/copy/t/177-320\endcsname{99}
\expandafter\def\csname R@nott/copy/t/33-80\endcsname{94}
\expandafter\def\csname R@nott/copy/t/81-176\endcsname{99}
\expandafter\def\csname R@nott/copy/t/all\endcsname{97}
\expandafter\def\csname R@nott/copybase/16\endcsname{0.573}
\expandafter\def\csname R@nott/copybase/16/gain\endcsname{83}
\expandafter\def\csname R@nott/copybase/16/matched\endcsname{71}
\expandafter\def\csname R@nott/copybase/backoff\endcsname{0.469}
\expandafter\def\csname R@nott/copybase/backoff/gain\endcsname{94}
\expandafter\def\csname R@nott/copybase/backoff/matched\endcsname{79}
\expandafter\def\csname R@nott/copybase/base\endcsname{1.391}
\expandafter\def\csname R@nott/copybase/m/bits_T336\endcsname{0.24}
\expandafter\def\csname R@nott/copybase/m/bits_T6\endcsname{1.41}
\expandafter\def\csname R@nott/copybase/m/bits_copy\endcsname{0.25}
\expandafter\def\csname R@nott/copybase/m/copy\endcsname{94}
\expandafter\def\csname R@nott/copybase/m/t336\endcsname{94}
\expandafter\def\csname R@nott/groups\endcsname{996}
\expandafter\def\csname R@nott/h32/copy\endcsname{98}
\expandafter\def\csname R@nott/h32/redshare/l\endcsname{81}
\expandafter\def\csname R@nott/h32/redshare/t\endcsname{74}
\expandafter\def\csname R@nott/h32/share\endcsname{60}
\expandafter\def\csname R@nott/h8/copy\endcsname{94}
\expandafter\def\csname R@nott/h8/redshare/l\endcsname{91}
\expandafter\def\csname R@nott/h8/redshare/t\endcsname{84}
\expandafter\def\csname R@nott/h8/share\endcsname{73}
\expandafter\def\csname R@nott/inview/18\endcsname{0.0}
\expandafter\def\csname R@nott/inview/192\endcsname{53.0}
\expandafter\def\csname R@nott/inview/336\endcsname{71.0}
\expandafter\def\csname R@nott/inview/48\endcsname{1.8}
\expandafter\def\csname R@nott/inview/6\endcsname{0.0}
\expandafter\def\csname R@nott/inview/96\endcsname{16.5}
\expandafter\def\csname R@nott/lag/l/18/1-32\endcsname{0.87}
\expandafter\def\csname R@nott/lag/l/18/177-320\endcsname{0.82}
\expandafter\def\csname R@nott/lag/l/18/33-80\endcsname{0.85}
\expandafter\def\csname R@nott/lag/l/18/81-176\endcsname{0.85}
\expandafter\def\csname R@nott/lag/l/18/held\endcsname{0.88}
\expandafter\def\csname R@nott/lag/l/18/none\endcsname{0.84}
\expandafter\def\csname R@nott/lag/l/192/1-32\endcsname{0.57}
\expandafter\def\csname R@nott/lag/l/192/177-320\endcsname{0.81}
\expandafter\def\csname R@nott/lag/l/192/33-80\endcsname{0.45}
\expandafter\def\csname R@nott/lag/l/192/81-176\endcsname{0.33}
\expandafter\def\csname R@nott/lag/l/192/held\endcsname{0.79}
\expandafter\def\csname R@nott/lag/l/192/none\endcsname{0.79}
\expandafter\def\csname R@nott/lag/l/336/1-32\endcsname{0.49}
\expandafter\def\csname R@nott/lag/l/336/177-320\endcsname{0.37}
\expandafter\def\csname R@nott/lag/l/336/33-80\endcsname{0.37}
\expandafter\def\csname R@nott/lag/l/336/81-176\endcsname{0.32}
\expandafter\def\csname R@nott/lag/l/336/held\endcsname{0.68}
\expandafter\def\csname R@nott/lag/l/336/none\endcsname{0.77}
\expandafter\def\csname R@nott/lag/l/48/1-32\endcsname{0.84}
\expandafter\def\csname R@nott/lag/l/48/177-320\endcsname{0.81}
\expandafter\def\csname R@nott/lag/l/48/33-80\endcsname{0.85}
\expandafter\def\csname R@nott/lag/l/48/81-176\endcsname{0.84}
\expandafter\def\csname R@nott/lag/l/48/held\endcsname{0.87}
\expandafter\def\csname R@nott/lag/l/48/none\endcsname{0.83}
\expandafter\def\csname R@nott/lag/l/6/1-32\endcsname{0.90}
\expandafter\def\csname R@nott/lag/l/6/177-320\endcsname{0.84}
\expandafter\def\csname R@nott/lag/l/6/33-80\endcsname{0.87}
\expandafter\def\csname R@nott/lag/l/6/81-176\endcsname{0.86}
\expandafter\def\csname R@nott/lag/l/6/held\endcsname{0.89}
\expandafter\def\csname R@nott/lag/l/6/none\endcsname{0.85}
\expandafter\def\csname R@nott/lag/l/96/1-32\endcsname{0.79}
\expandafter\def\csname R@nott/lag/l/96/177-320\endcsname{0.79}
\expandafter\def\csname R@nott/lag/l/96/33-80\endcsname{0.65}
\expandafter\def\csname R@nott/lag/l/96/81-176\endcsname{0.80}
\expandafter\def\csname R@nott/lag/l/96/held\endcsname{0.85}
\expandafter\def\csname R@nott/lag/l/96/none\endcsname{0.81}
\expandafter\def\csname R@nott/lag/t/18/1-32\endcsname{1.88}
\expandafter\def\csname R@nott/lag/t/18/177-320\endcsname{1.31}
\expandafter\def\csname R@nott/lag/t/18/33-80\endcsname{1.55}
\expandafter\def\csname R@nott/lag/t/18/81-176\endcsname{1.46}
\expandafter\def\csname R@nott/lag/t/18/held\endcsname{2.36}
\expandafter\def\csname R@nott/lag/t/18/none\endcsname{1.39}
\expandafter\def\csname R@nott/lag/t/192/1-32\endcsname{0.65}
\expandafter\def\csname R@nott/lag/t/192/177-320\endcsname{0.96}
\expandafter\def\csname R@nott/lag/t/192/33-80\endcsname{0.24}
\expandafter\def\csname R@nott/lag/t/192/81-176\endcsname{0.20}
\expandafter\def\csname R@nott/lag/t/192/held\endcsname{1.33}
\expandafter\def\csname R@nott/lag/t/192/none\endcsname{0.93}
\expandafter\def\csname R@nott/lag/t/336/1-32\endcsname{0.42}
\expandafter\def\csname R@nott/lag/t/336/177-320\endcsname{0.18}
\expandafter\def\csname R@nott/lag/t/336/33-80\endcsname{0.22}
\expandafter\def\csname R@nott/lag/t/336/81-176\endcsname{0.17}
\expandafter\def\csname R@nott/lag/t/336/held\endcsname{0.90}
\expandafter\def\csname R@nott/lag/t/336/none\endcsname{0.93}
\expandafter\def\csname R@nott/lag/t/48/1-32\endcsname{1.93}
\expandafter\def\csname R@nott/lag/t/48/177-320\endcsname{1.39}
\expandafter\def\csname R@nott/lag/t/48/33-80\endcsname{1.70}
\expandafter\def\csname R@nott/lag/t/48/81-176\endcsname{1.54}
\expandafter\def\csname R@nott/lag/t/48/held\endcsname{2.29}
\expandafter\def\csname R@nott/lag/t/48/none\endcsname{1.47}
\expandafter\def\csname R@nott/lag/t/6/1-32\endcsname{1.81}
\expandafter\def\csname R@nott/lag/t/6/177-320\endcsname{1.24}
\expandafter\def\csname R@nott/lag/t/6/33-80\endcsname{1.49}
\expandafter\def\csname R@nott/lag/t/6/81-176\endcsname{1.42}
\expandafter\def\csname R@nott/lag/t/6/held\endcsname{2.40}
\expandafter\def\csname R@nott/lag/t/6/none\endcsname{1.35}
\expandafter\def\csname R@nott/lag/t/96/1-32\endcsname{1.49}
\expandafter\def\csname R@nott/lag/t/96/177-320\endcsname{1.26}
\expandafter\def\csname R@nott/lag/t/96/33-80\endcsname{0.99}
\expandafter\def\csname R@nott/lag/t/96/81-176\endcsname{1.34}
\expandafter\def\csname R@nott/lag/t/96/held\endcsname{2.04}
\expandafter\def\csname R@nott/lag/t/96/none\endcsname{1.32}
\expandafter\def\csname R@nott/lat/0\endcsname{0.958}
\expandafter\def\csname R@nott/lat/0/n\endcsname{1}
\expandafter\def\csname R@nott/lat/0/pertoken\endcsname{10.22}
\expandafter\def\csname R@nott/lat/18\endcsname{0.842}
\expandafter\def\csname R@nott/lat/18/ep/max\endcsname{82}
\expandafter\def\csname R@nott/lat/18/ep/min\endcsname{51}
\expandafter\def\csname R@nott/lat/18/n\endcsname{3}
\expandafter\def\csname R@nott/lat/18/pertoken\endcsname{8.98}
\expandafter\def\csname R@nott/lat/18/sd\endcsname{0.002}
\expandafter\def\csname R@nott/lat/192\endcsname{0.571}
\expandafter\def\csname R@nott/lat/192/ep/max\endcsname{177}
\expandafter\def\csname R@nott/lat/192/ep/min\endcsname{99}
\expandafter\def\csname R@nott/lat/192/n\endcsname{3}
\expandafter\def\csname R@nott/lat/192/pertoken\endcsname{6.09}
\expandafter\def\csname R@nott/lat/192/sd\endcsname{0.015}
\expandafter\def\csname R@nott/lat/336\endcsname{0.465}
\expandafter\def\csname R@nott/lat/336/ep/max\endcsname{131}
\expandafter\def\csname R@nott/lat/336/ep/min\endcsname{95}
\expandafter\def\csname R@nott/lat/336/n\endcsname{3}
\expandafter\def\csname R@nott/lat/336/pertoken\endcsname{4.96}
\expandafter\def\csname R@nott/lat/336/sd\endcsname{0.009}
\expandafter\def\csname R@nott/lat/48\endcsname{0.834}
\expandafter\def\csname R@nott/lat/48/ep/max\endcsname{97}
\expandafter\def\csname R@nott/lat/48/ep/min\endcsname{63}
\expandafter\def\csname R@nott/lat/48/n\endcsname{3}
\expandafter\def\csname R@nott/lat/48/pertoken\endcsname{8.90}
\expandafter\def\csname R@nott/lat/48/sd\endcsname{0.005}
\expandafter\def\csname R@nott/lat/6\endcsname{0.857}
\expandafter\def\csname R@nott/lat/6/ep/max\endcsname{69}
\expandafter\def\csname R@nott/lat/6/ep/min\endcsname{28}
\expandafter\def\csname R@nott/lat/6/n\endcsname{3}
\expandafter\def\csname R@nott/lat/6/pertoken\endcsname{9.14}
\expandafter\def\csname R@nott/lat/6/sd\endcsname{0.002}
\expandafter\def\csname R@nott/lat/96\endcsname{0.775}
\expandafter\def\csname R@nott/lat/96/ep/max\endcsname{118}
\expandafter\def\csname R@nott/lat/96/ep/min\endcsname{115}
\expandafter\def\csname R@nott/lat/96/n\endcsname{3}
\expandafter\def\csname R@nott/lat/96/pertoken\endcsname{8.27}
\expandafter\def\csname R@nott/lat/96/sd\endcsname{0.004}
\expandafter\def\csname R@nott/lat/drop\endcsname{46}
\expandafter\def\csname R@nott/lat/ep/max\endcsname{177}
\expandafter\def\csname R@nott/lat/maxsd\endcsname{0.015}
\expandafter\def\csname R@nott/leak/test/verbatim\endcsname{0.0}
\expandafter\def\csname R@nott/lenratio\endcsname{1.64}
\expandafter\def\csname R@nott/longep/max\endcsname{178}
\expandafter\def\csname R@nott/longep/min\endcsname{95}
\expandafter\def\csname R@nott/moved\endcsname{4}
\expandafter\def\csname R@nott/pieces/all\endcsname{1033}
\expandafter\def\csname R@nott/pieces/test\endcsname{154}
\expandafter\def\csname R@nott/pieces/testwin\endcsname{133}
\expandafter\def\csname R@nott/pieces/train\endcsname{729}
\expandafter\def\csname R@nott/pieces/val\endcsname{150}
\expandafter\def\csname R@nott/pitchlo\endcsname{42}
\expandafter\def\csname R@nott/reached/l/18\endcsname{4}
\expandafter\def\csname R@nott/reached/l/192\endcsname{73}
\expandafter\def\csname R@nott/reached/l/336\endcsname{100}
\expandafter\def\csname R@nott/reached/l/48\endcsname{6}
\expandafter\def\csname R@nott/reached/l/6\endcsname{0}
\expandafter\def\csname R@nott/reached/l/96\endcsname{21}
\expandafter\def\csname R@nott/reached/t/18\endcsname{-5}
\expandafter\def\csname R@nott/reached/t/192\endcsname{84}
\expandafter\def\csname R@nott/reached/t/336\endcsname{100}
\expandafter\def\csname R@nott/reached/t/48\endcsname{-14}
\expandafter\def\csname R@nott/reached/t/6\endcsname{0}
\expandafter\def\csname R@nott/reached/t/96\endcsname{12}
\expandafter\def\csname R@nott/redshare/l/none\endcsname{6}
\expandafter\def\csname R@nott/redshare/l/repeat\endcsname{93}
\expandafter\def\csname R@nott/redshare/t/none\endcsname{12}
\expandafter\def\csname R@nott/redshare/t/repeat\endcsname{87}
\expandafter\def\csname R@nott/rest\endcsname{1.7}
\expandafter\def\csname R@nott/sel/dropped/median\endcsname{268}
\expandafter\def\csname R@nott/sel/dropped/n\endcsname{21}
\expandafter\def\csname R@nott/sel/dropped/repeat\endcsname{42}
\expandafter\def\csname R@nott/sel/dropped/repeat256\endcsname{42}
\expandafter\def\csname R@nott/sel/kept/median\endcsname{524}
\expandafter\def\csname R@nott/sel/kept/n\endcsname{133}
\expandafter\def\csname R@nott/sel/kept/repeat\endcsname{55}
\expandafter\def\csname R@nott/sel/kept/repeat256\endcsname{41}
\expandafter\def\csname R@nott/share/s/1-32\endcsname{1.9}
\expandafter\def\csname R@nott/share/s/177-320\endcsname{17.7}
\expandafter\def\csname R@nott/share/s/33-80\endcsname{15.4}
\expandafter\def\csname R@nott/share/s/81-176\endcsname{36.4}
\expandafter\def\csname R@nott/share/s/held\endcsname{1.2}
\expandafter\def\csname R@nott/share/s/none\endcsname{27.5}
\expandafter\def\csname R@nott/share/s/repeat\endcsname{71}
\expandafter\def\csname R@nott/share/t/1-32\endcsname{1.8}
\expandafter\def\csname R@nott/share/t/177-320\endcsname{17.9}
\expandafter\def\csname R@nott/share/t/33-80\endcsname{14.7}
\expandafter\def\csname R@nott/share/t/81-176\endcsname{36.6}
\expandafter\def\csname R@nott/share/t/held\endcsname{0.7}
\expandafter\def\csname R@nott/share/t/none\endcsname{28.3}
\expandafter\def\csname R@nott/share/t/repeat\endcsname{71}
\expandafter\def\csname R@nott/targets\endcsname{48}
\expandafter\def\csname R@nott/tok/0\endcsname{4.366}
\expandafter\def\csname R@nott/tok/0/n\endcsname{1}
\expandafter\def\csname R@nott/tok/18\endcsname{1.440}
\expandafter\def\csname R@nott/tok/18/ep/max\endcsname{83}
\expandafter\def\csname R@nott/tok/18/ep/min\endcsname{63}
\expandafter\def\csname R@nott/tok/18/n\endcsname{3}
\expandafter\def\csname R@nott/tok/18/sd\endcsname{0.021}
\expandafter\def\csname R@nott/tok/192\endcsname{0.567}
\expandafter\def\csname R@nott/tok/192/ep/max\endcsname{178}
\expandafter\def\csname R@nott/tok/192/ep/min\endcsname{114}
\expandafter\def\csname R@nott/tok/192/n\endcsname{3}
\expandafter\def\csname R@nott/tok/192/sd\endcsname{0.008}
\expandafter\def\csname R@nott/tok/336\endcsname{0.405}
\expandafter\def\csname R@nott/tok/336/ep/max\endcsname{171}
\expandafter\def\csname R@nott/tok/336/ep/min\endcsname{104}
\expandafter\def\csname R@nott/tok/336/n\endcsname{3}
\expandafter\def\csname R@nott/tok/336/sd\endcsname{0.006}
\expandafter\def\csname R@nott/tok/48\endcsname{1.529}
\expandafter\def\csname R@nott/tok/48/ep/max\endcsname{60}
\expandafter\def\csname R@nott/tok/48/ep/min\endcsname{43}
\expandafter\def\csname R@nott/tok/48/n\endcsname{3}
\expandafter\def\csname R@nott/tok/48/sd\endcsname{0.090}
\expandafter\def\csname R@nott/tok/6\endcsname{1.391}
\expandafter\def\csname R@nott/tok/6/ep/max\endcsname{94}
\expandafter\def\csname R@nott/tok/6/ep/min\endcsname{35}
\expandafter\def\csname R@nott/tok/6/n\endcsname{3}
\expandafter\def\csname R@nott/tok/6/sd\endcsname{0.015}
\expandafter\def\csname R@nott/tok/96\endcsname{1.274}
\expandafter\def\csname R@nott/tok/96/ep/max\endcsname{164}
\expandafter\def\csname R@nott/tok/96/ep/min\endcsname{29}
\expandafter\def\csname R@nott/tok/96/n\endcsname{3}
\expandafter\def\csname R@nott/tok/96/sd\endcsname{0.326}
\expandafter\def\csname R@nott/tok/drop\endcsname{71}
\expandafter\def\csname R@nott/tok/ep/max\endcsname{178}
\expandafter\def\csname R@nott/tok/maxsd\endcsname{0.326}
\expandafter\def\csname R@nott/tokens/test\endcsname{84{,}466}
\expandafter\def\csname R@nott/tokens/train\endcsname{382{,}037}
\expandafter\def\csname R@nott/tokens/val\endcsname{90{,}260}
\expandafter\def\csname R@nott/trans/copy\endcsname{79}
\expandafter\def\csname R@nott/trans/other/336\endcsname{0.93}
\expandafter\def\csname R@nott/trans/other/6\endcsname{1.34}
\expandafter\def\csname R@nott/trans/share\endcsname{0.9}
\expandafter\def\csname R@nott/trans/t/336\endcsname{1.08}
\expandafter\def\csname R@nott/trans/t/6\endcsname{1.66}
\expandafter\def\csname R@nott/v5/0\endcsname{0.958}
\expandafter\def\csname R@nott/v5/0/n\endcsname{1}
\expandafter\def\csname R@nott/v5/18\endcsname{0.852}
\expandafter\def\csname R@nott/v5/18/ep/max\endcsname{77}
\expandafter\def\csname R@nott/v5/18/ep/min\endcsname{44}
\expandafter\def\csname R@nott/v5/18/n\endcsname{3}
\expandafter\def\csname R@nott/v5/18/sd\endcsname{0.001}
\expandafter\def\csname R@nott/v5/192\endcsname{0.886}
\expandafter\def\csname R@nott/v5/192/ep/max\endcsname{67}
\expandafter\def\csname R@nott/v5/192/ep/min\endcsname{22}
\expandafter\def\csname R@nott/v5/192/n\endcsname{3}
\expandafter\def\csname R@nott/v5/192/sd\endcsname{0.001}
\expandafter\def\csname R@nott/v5/336\endcsname{0.891}
\expandafter\def\csname R@nott/v5/336/ep/max\endcsname{81}
\expandafter\def\csname R@nott/v5/336/ep/min\endcsname{17}
\expandafter\def\csname R@nott/v5/336/n\endcsname{3}
\expandafter\def\csname R@nott/v5/336/sd\endcsname{0.001}
\expandafter\def\csname R@nott/v5/48\endcsname{0.843}
\expandafter\def\csname R@nott/v5/48/ep/max\endcsname{90}
\expandafter\def\csname R@nott/v5/48/ep/min\endcsname{74}
\expandafter\def\csname R@nott/v5/48/n\endcsname{3}
\expandafter\def\csname R@nott/v5/48/sd\endcsname{0.004}
\expandafter\def\csname R@nott/v5/6\endcsname{0.856}
\expandafter\def\csname R@nott/v5/6/ep/max\endcsname{89}
\expandafter\def\csname R@nott/v5/6/ep/min\endcsname{49}
\expandafter\def\csname R@nott/v5/6/n\endcsname{3}
\expandafter\def\csname R@nott/v5/6/sd\endcsname{0.000}
\expandafter\def\csname R@nott/v5/96\endcsname{0.891}
\expandafter\def\csname R@nott/v5/96/ep/max\endcsname{58}
\expandafter\def\csname R@nott/v5/96/ep/min\endcsname{33}
\expandafter\def\csname R@nott/v5/96/n\endcsname{3}
\expandafter\def\csname R@nott/v5/96/sd\endcsname{0.001}
\expandafter\def\csname R@nott/v5/ep/max\endcsname{90}
\expandafter\def\csname R@nott/v5/maxsd\endcsname{0.004}
\expandafter\def\csname R@nott/win/test\endcsname{660}
\expandafter\def\csname R@nott/win/train\endcsname{2789}
\expandafter\def\csname R@nott/window\endcsname{384}
\expandafter\def\csname R@nottnoaug/ae/acc\endcsname{99.691}
\expandafter\def\csname R@nottnoaug/lat/0\endcsname{0.988}
\expandafter\def\csname R@nottnoaug/lat/0/n\endcsname{1}
\expandafter\def\csname R@nottnoaug/lat/18\endcsname{0.914}
\expandafter\def\csname R@nottnoaug/lat/18/ep/max\endcsname{6}
\expandafter\def\csname R@nottnoaug/lat/18/ep/min\endcsname{3}
\expandafter\def\csname R@nottnoaug/lat/18/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/lat/18/sd\endcsname{0.001}
\expandafter\def\csname R@nottnoaug/lat/192\endcsname{0.770}
\expandafter\def\csname R@nottnoaug/lat/192/ep/max\endcsname{15}
\expandafter\def\csname R@nottnoaug/lat/192/ep/min\endcsname{14}
\expandafter\def\csname R@nottnoaug/lat/192/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/lat/192/sd\endcsname{0.004}
\expandafter\def\csname R@nottnoaug/lat/336\endcsname{0.632}
\expandafter\def\csname R@nottnoaug/lat/336/ep/max\endcsname{24}
\expandafter\def\csname R@nottnoaug/lat/336/ep/min\endcsname{18}
\expandafter\def\csname R@nottnoaug/lat/336/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/lat/336/sd\endcsname{0.005}
\expandafter\def\csname R@nottnoaug/lat/48\endcsname{0.914}
\expandafter\def\csname R@nottnoaug/lat/48/ep/max\endcsname{3}
\expandafter\def\csname R@nottnoaug/lat/48/ep/min\endcsname{2}
\expandafter\def\csname R@nottnoaug/lat/48/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/lat/48/sd\endcsname{0.003}
\expandafter\def\csname R@nottnoaug/lat/6\endcsname{0.913}
\expandafter\def\csname R@nottnoaug/lat/6/ep/max\endcsname{7}
\expandafter\def\csname R@nottnoaug/lat/6/ep/min\endcsname{5}
\expandafter\def\csname R@nottnoaug/lat/6/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/lat/6/sd\endcsname{0.001}
\expandafter\def\csname R@nottnoaug/lat/96\endcsname{0.911}
\expandafter\def\csname R@nottnoaug/lat/96/ep/max\endcsname{4}
\expandafter\def\csname R@nottnoaug/lat/96/ep/min\endcsname{1}
\expandafter\def\csname R@nottnoaug/lat/96/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/lat/96/sd\endcsname{0.003}
\expandafter\def\csname R@nottnoaug/lat/drop\endcsname{31}
\expandafter\def\csname R@nottnoaug/lat/ep/max\endcsname{24}
\expandafter\def\csname R@nottnoaug/lat/maxsd\endcsname{0.005}
\expandafter\def\csname R@nottnoaug/longep/max\endcsname{24}
\expandafter\def\csname R@nottnoaug/longep/min\endcsname{11}
\expandafter\def\csname R@nottnoaug/tok/0\endcsname{3.894}
\expandafter\def\csname R@nottnoaug/tok/0/n\endcsname{1}
\expandafter\def\csname R@nottnoaug/tok/18\endcsname{1.516}
\expandafter\def\csname R@nottnoaug/tok/18/ep/max\endcsname{12}
\expandafter\def\csname R@nottnoaug/tok/18/ep/min\endcsname{11}
\expandafter\def\csname R@nottnoaug/tok/18/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/tok/18/sd\endcsname{0.013}
\expandafter\def\csname R@nottnoaug/tok/192\endcsname{1.151}
\expandafter\def\csname R@nottnoaug/tok/192/ep/max\endcsname{14}
\expandafter\def\csname R@nottnoaug/tok/192/ep/min\endcsname{12}
\expandafter\def\csname R@nottnoaug/tok/192/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/tok/192/sd\endcsname{0.018}
\expandafter\def\csname R@nottnoaug/tok/336\endcsname{0.805}
\expandafter\def\csname R@nottnoaug/tok/336/ep/max\endcsname{21}
\expandafter\def\csname R@nottnoaug/tok/336/ep/min\endcsname{11}
\expandafter\def\csname R@nottnoaug/tok/336/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/tok/336/sd\endcsname{0.252}
\expandafter\def\csname R@nottnoaug/tok/48\endcsname{1.491}
\expandafter\def\csname R@nottnoaug/tok/48/ep/max\endcsname{17}
\expandafter\def\csname R@nottnoaug/tok/48/ep/min\endcsname{12}
\expandafter\def\csname R@nottnoaug/tok/48/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/tok/48/sd\endcsname{0.154}
\expandafter\def\csname R@nottnoaug/tok/6\endcsname{1.393}
\expandafter\def\csname R@nottnoaug/tok/6/ep/max\endcsname{22}
\expandafter\def\csname R@nottnoaug/tok/6/ep/min\endcsname{20}
\expandafter\def\csname R@nottnoaug/tok/6/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/tok/6/sd\endcsname{0.004}
\expandafter\def\csname R@nottnoaug/tok/96\endcsname{1.091}
\expandafter\def\csname R@nottnoaug/tok/96/ep/max\endcsname{22}
\expandafter\def\csname R@nottnoaug/tok/96/ep/min\endcsname{11}
\expandafter\def\csname R@nottnoaug/tok/96/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/tok/96/sd\endcsname{0.020}
\expandafter\def\csname R@nottnoaug/tok/drop\endcsname{42}
\expandafter\def\csname R@nottnoaug/tok/ep/max\endcsname{22}
\expandafter\def\csname R@nottnoaug/tok/maxsd\endcsname{0.252}
\expandafter\def\csname R@nottnoaug/v5/0\endcsname{0.988}
\expandafter\def\csname R@nottnoaug/v5/0/n\endcsname{1}
\expandafter\def\csname R@nottnoaug/v5/18\endcsname{0.942}
\expandafter\def\csname R@nottnoaug/v5/18/ep/max\endcsname{8}
\expandafter\def\csname R@nottnoaug/v5/18/ep/min\endcsname{4}
\expandafter\def\csname R@nottnoaug/v5/18/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/v5/18/sd\endcsname{0.002}
\expandafter\def\csname R@nottnoaug/v5/192\endcsname{0.948}
\expandafter\def\csname R@nottnoaug/v5/192/ep/max\endcsname{11}
\expandafter\def\csname R@nottnoaug/v5/192/ep/min\endcsname{6}
\expandafter\def\csname R@nottnoaug/v5/192/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/v5/192/sd\endcsname{0.001}
\expandafter\def\csname R@nottnoaug/v5/336\endcsname{0.952}
\expandafter\def\csname R@nottnoaug/v5/336/ep/max\endcsname{15}
\expandafter\def\csname R@nottnoaug/v5/336/ep/min\endcsname{5}
\expandafter\def\csname R@nottnoaug/v5/336/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/v5/336/sd\endcsname{0.001}
\expandafter\def\csname R@nottnoaug/v5/48\endcsname{0.957}
\expandafter\def\csname R@nottnoaug/v5/48/ep/max\endcsname{7}
\expandafter\def\csname R@nottnoaug/v5/48/ep/min\endcsname{2}
\expandafter\def\csname R@nottnoaug/v5/48/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/v5/48/sd\endcsname{0.001}
\expandafter\def\csname R@nottnoaug/v5/6\endcsname{0.913}
\expandafter\def\csname R@nottnoaug/v5/6/ep/max\endcsname{8}
\expandafter\def\csname R@nottnoaug/v5/6/ep/min\endcsname{6}
\expandafter\def\csname R@nottnoaug/v5/6/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/v5/6/sd\endcsname{0.001}
\expandafter\def\csname R@nottnoaug/v5/96\endcsname{0.952}
\expandafter\def\csname R@nottnoaug/v5/96/ep/max\endcsname{6}
\expandafter\def\csname R@nottnoaug/v5/96/ep/min\endcsname{4}
\expandafter\def\csname R@nottnoaug/v5/96/n\endcsname{3}
\expandafter\def\csname R@nottnoaug/v5/96/sd\endcsname{0.001}
\expandafter\def\csname R@nottnoaug/v5/ep/max\endcsname{15}
\expandafter\def\csname R@nottnoaug/v5/maxsd\endcsname{0.002}
\expandafter\def\csname R@nottv2/lat/0\endcsname{0.964}
\expandafter\def\csname R@nottv2/lat/0/n\endcsname{1}
\expandafter\def\csname R@nottv2/lat/18\endcsname{0.807}
\expandafter\def\csname R@nottv2/lat/18/ep/max\endcsname{5}
\expandafter\def\csname R@nottv2/lat/18/ep/min\endcsname{2}
\expandafter\def\csname R@nottv2/lat/18/n\endcsname{3}
\expandafter\def\csname R@nottv2/lat/18/sd\endcsname{0.002}
\expandafter\def\csname R@nottv2/lat/192\endcsname{0.783}
\expandafter\def\csname R@nottv2/lat/192/ep/max\endcsname{4}
\expandafter\def\csname R@nottv2/lat/192/ep/min\endcsname{3}
\expandafter\def\csname R@nottv2/lat/192/n\endcsname{3}
\expandafter\def\csname R@nottv2/lat/192/sd\endcsname{0.001}
\expandafter\def\csname R@nottv2/lat/336\endcsname{0.724}
\expandafter\def\csname R@nottv2/lat/336/ep/max\endcsname{8}
\expandafter\def\csname R@nottv2/lat/336/ep/min\endcsname{6}
\expandafter\def\csname R@nottv2/lat/336/n\endcsname{3}
\expandafter\def\csname R@nottv2/lat/336/sd\endcsname{0.011}
\expandafter\def\csname R@nottv2/lat/48\endcsname{0.807}
\expandafter\def\csname R@nottv2/lat/48/ep/max\endcsname{4}
\expandafter\def\csname R@nottv2/lat/48/ep/min\endcsname{2}
\expandafter\def\csname R@nottv2/lat/48/n\endcsname{3}
\expandafter\def\csname R@nottv2/lat/48/sd\endcsname{0.001}
\expandafter\def\csname R@nottv2/lat/6\endcsname{0.803}
\expandafter\def\csname R@nottv2/lat/6/ep/max\endcsname{7}
\expandafter\def\csname R@nottv2/lat/6/ep/min\endcsname{5}
\expandafter\def\csname R@nottv2/lat/6/n\endcsname{3}
\expandafter\def\csname R@nottv2/lat/6/sd\endcsname{0.000}
\expandafter\def\csname R@nottv2/lat/96\endcsname{0.805}
\expandafter\def\csname R@nottv2/lat/96/ep/max\endcsname{4}
\expandafter\def\csname R@nottv2/lat/96/ep/min\endcsname{2}
\expandafter\def\csname R@nottv2/lat/96/n\endcsname{3}
\expandafter\def\csname R@nottv2/lat/96/sd\endcsname{0.001}
\expandafter\def\csname R@nottv2/lat/drop\endcsname{10}
\expandafter\def\csname R@nottv2/lat/ep/max\endcsname{8}
\expandafter\def\csname R@nottv2/lat/maxsd\endcsname{0.011}
\expandafter\def\csname R@nottv2/longep/max\endcsname{14}
\expandafter\def\csname R@nottv2/longep/min\endcsname{3}
\expandafter\def\csname R@nottv2/tok/0\endcsname{3.860}
\expandafter\def\csname R@nottv2/tok/0/n\endcsname{1}
\expandafter\def\csname R@nottv2/tok/18\endcsname{1.211}
\expandafter\def\csname R@nottv2/tok/18/ep/max\endcsname{6}
\expandafter\def\csname R@nottv2/tok/18/ep/min\endcsname{4}
\expandafter\def\csname R@nottv2/tok/18/n\endcsname{3}
\expandafter\def\csname R@nottv2/tok/18/sd\endcsname{0.002}
\expandafter\def\csname R@nottv2/tok/192\endcsname{1.041}
\expandafter\def\csname R@nottv2/tok/192/ep/max\endcsname{7}
\expandafter\def\csname R@nottv2/tok/192/ep/min\endcsname{7}
\expandafter\def\csname R@nottv2/tok/192/n\endcsname{3}
\expandafter\def\csname R@nottv2/tok/192/sd\endcsname{0.007}
\expandafter\def\csname R@nottv2/tok/336\endcsname{0.840}
\expandafter\def\csname R@nottv2/tok/336/ep/max\endcsname{14}
\expandafter\def\csname R@nottv2/tok/336/ep/min\endcsname{9}
\expandafter\def\csname R@nottv2/tok/336/n\endcsname{3}
\expandafter\def\csname R@nottv2/tok/336/sd\endcsname{0.015}
\expandafter\def\csname R@nottv2/tok/48\endcsname{1.208}
\expandafter\def\csname R@nottv2/tok/48/ep/max\endcsname{6}
\expandafter\def\csname R@nottv2/tok/48/ep/min\endcsname{3}
\expandafter\def\csname R@nottv2/tok/48/n\endcsname{3}
\expandafter\def\csname R@nottv2/tok/48/sd\endcsname{0.003}
\expandafter\def\csname R@nottv2/tok/6\endcsname{1.223}
\expandafter\def\csname R@nottv2/tok/6/ep/max\endcsname{51}
\expandafter\def\csname R@nottv2/tok/6/ep/min\endcsname{22}
\expandafter\def\csname R@nottv2/tok/6/n\endcsname{3}
\expandafter\def\csname R@nottv2/tok/6/sd\endcsname{0.001}
\expandafter\def\csname R@nottv2/tok/96\endcsname{1.198}
\expandafter\def\csname R@nottv2/tok/96/ep/max\endcsname{5}
\expandafter\def\csname R@nottv2/tok/96/ep/min\endcsname{3}
\expandafter\def\csname R@nottv2/tok/96/n\endcsname{3}
\expandafter\def\csname R@nottv2/tok/96/sd\endcsname{0.004}
\expandafter\def\csname R@nottv2/tok/drop\endcsname{31}
\expandafter\def\csname R@nottv2/tok/ep/max\endcsname{51}
\expandafter\def\csname R@nottv2/tok/maxsd\endcsname{0.015}
\expandafter\def\csname R@nottv2/v5/0\endcsname{0.964}
\expandafter\def\csname R@nottv2/v5/0/n\endcsname{1}
\expandafter\def\csname R@nottv2/v5/18\endcsname{0.805}
\expandafter\def\csname R@nottv2/v5/18/ep/max\endcsname{6}
\expandafter\def\csname R@nottv2/v5/18/ep/min\endcsname{5}
\expandafter\def\csname R@nottv2/v5/18/n\endcsname{3}
\expandafter\def\csname R@nottv2/v5/18/sd\endcsname{0.002}
\expandafter\def\csname R@nottv2/v5/192\endcsname{0.923}
\expandafter\def\csname R@nottv2/v5/192/ep/max\endcsname{7}
\expandafter\def\csname R@nottv2/v5/192/ep/min\endcsname{4}
\expandafter\def\csname R@nottv2/v5/192/n\endcsname{3}
\expandafter\def\csname R@nottv2/v5/192/sd\endcsname{0.001}
\expandafter\def\csname R@nottv2/v5/336\endcsname{0.928}
\expandafter\def\csname R@nottv2/v5/336/ep/max\endcsname{8}
\expandafter\def\csname R@nottv2/v5/336/ep/min\endcsname{3}
\expandafter\def\csname R@nottv2/v5/336/n\endcsname{3}
\expandafter\def\csname R@nottv2/v5/336/sd\endcsname{0.000}
\expandafter\def\csname R@nottv2/v5/48\endcsname{0.802}
\expandafter\def\csname R@nottv2/v5/48/ep/max\endcsname{6}
\expandafter\def\csname R@nottv2/v5/48/ep/min\endcsname{4}
\expandafter\def\csname R@nottv2/v5/48/n\endcsname{3}
\expandafter\def\csname R@nottv2/v5/48/sd\endcsname{0.002}
\expandafter\def\csname R@nottv2/v5/6\endcsname{0.804}
\expandafter\def\csname R@nottv2/v5/6/ep/max\endcsname{7}
\expandafter\def\csname R@nottv2/v5/6/ep/min\endcsname{4}
\expandafter\def\csname R@nottv2/v5/6/n\endcsname{3}
\expandafter\def\csname R@nottv2/v5/6/sd\endcsname{0.001}
\expandafter\def\csname R@nottv2/v5/96\endcsname{0.800}
\expandafter\def\csname R@nottv2/v5/96/ep/max\endcsname{7}
\expandafter\def\csname R@nottv2/v5/96/ep/min\endcsname{6}
\expandafter\def\csname R@nottv2/v5/96/n\endcsname{3}
\expandafter\def\csname R@nottv2/v5/96/sd\endcsname{0.001}
\expandafter\def\csname R@nottv2/v5/ep/max\endcsname{8}
\expandafter\def\csname R@nottv2/v5/maxsd\endcsname{0.002}
\expandafter\def\csname R@old/jsb/neardup\endcsname{3.2}
\expandafter\def\csname R@old/jsb/verbatim\endcsname{1.2}
\expandafter\def\csname R@old/maestro/composition\endcsname{99.8}
\expandafter\def\csname R@old/maestro/neardup\endcsname{0.0}
\expandafter\def\csname R@old/maestro/performance\endcsname{99.6}
\expandafter\def\csname R@old/maestro/verbatim\endcsname{1.7}
\expandafter\def\csname R@old/musicnet/neardup\endcsname{16.9}
\expandafter\def\csname R@old/musicnet/recording\endcsname{100}
\expandafter\def\csname R@old/musicnet/verbatim\endcsname{19.8}
\expandafter\def\csname R@old/nottingham/neardup\endcsname{51.5}
\expandafter\def\csname R@old/nottingham/tune\endcsname{92.4}
\expandafter\def\csname R@old/nottingham/verbatim\endcsname{58.4}
\expandafter\def\csname R@oneill/abl/l/repl/18\endcsname{0.932}
\expandafter\def\csname R@oneill/abl/l/repl/18/none\endcsname{0.913}
\expandafter\def\csname R@oneill/abl/l/repl/18/repeat\endcsname{0.939}
\expandafter\def\csname R@oneill/abl/l/repl/192\endcsname{0.596}
\expandafter\def\csname R@oneill/abl/l/repl/192/none\endcsname{0.716}
\expandafter\def\csname R@oneill/abl/l/repl/192/repeat\endcsname{0.555}
\expandafter\def\csname R@oneill/abl/l/repl/48\endcsname{0.889}
\expandafter\def\csname R@oneill/abl/l/repl/48/none\endcsname{0.875}
\expandafter\def\csname R@oneill/abl/l/repl/48/repeat\endcsname{0.894}
\expandafter\def\csname R@oneill/abl/l/repl/6\endcsname{0.945}
\expandafter\def\csname R@oneill/abl/l/repl/6/none\endcsname{0.932}
\expandafter\def\csname R@oneill/abl/l/repl/6/repeat\endcsname{0.949}
\expandafter\def\csname R@oneill/abl/l/repl/96\endcsname{0.767}
\expandafter\def\csname R@oneill/abl/l/repl/96/none\endcsname{0.794}
\expandafter\def\csname R@oneill/abl/l/repl/96/repeat\endcsname{0.757}
\expandafter\def\csname R@oneill/abl/l/trunc/18\endcsname{1.253}
\expandafter\def\csname R@oneill/abl/l/trunc/18/none\endcsname{1.155}
\expandafter\def\csname R@oneill/abl/l/trunc/18/repeat\endcsname{1.286}
\expandafter\def\csname R@oneill/abl/l/trunc/192\endcsname{0.595}
\expandafter\def\csname R@oneill/abl/l/trunc/192/none\endcsname{0.719}
\expandafter\def\csname R@oneill/abl/l/trunc/192/repeat\endcsname{0.553}
\expandafter\def\csname R@oneill/abl/l/trunc/336\endcsname{0.419}
\expandafter\def\csname R@oneill/abl/l/trunc/336/none\endcsname{0.680}
\expandafter\def\csname R@oneill/abl/l/trunc/336/repeat\endcsname{0.329}
\expandafter\def\csname R@oneill/abl/l/trunc/48\endcsname{0.947}
\expandafter\def\csname R@oneill/abl/l/trunc/48/none\endcsname{0.912}
\expandafter\def\csname R@oneill/abl/l/trunc/48/repeat\endcsname{0.959}
\expandafter\def\csname R@oneill/abl/l/trunc/6\endcsname{1.815}
\expandafter\def\csname R@oneill/abl/l/trunc/6/none\endcsname{1.764}
\expandafter\def\csname R@oneill/abl/l/trunc/6/repeat\endcsname{1.833}
\expandafter\def\csname R@oneill/abl/l/trunc/96\endcsname{0.749}
\expandafter\def\csname R@oneill/abl/l/trunc/96/none\endcsname{0.793}
\expandafter\def\csname R@oneill/abl/l/trunc/96/repeat\endcsname{0.733}
\expandafter\def\csname R@oneill/abl/t/repl/18\endcsname{2.232}
\expandafter\def\csname R@oneill/abl/t/repl/18/none\endcsname{2.208}
\expandafter\def\csname R@oneill/abl/t/repl/18/repeat\endcsname{2.240}
\expandafter\def\csname R@oneill/abl/t/repl/192\endcsname{0.877}
\expandafter\def\csname R@oneill/abl/t/repl/192/none\endcsname{1.353}
\expandafter\def\csname R@oneill/abl/t/repl/192/repeat\endcsname{0.704}
\expandafter\def\csname R@oneill/abl/t/repl/48\endcsname{1.956}
\expandafter\def\csname R@oneill/abl/t/repl/48/none\endcsname{1.981}
\expandafter\def\csname R@oneill/abl/t/repl/48/repeat\endcsname{1.947}
\expandafter\def\csname R@oneill/abl/t/repl/6\endcsname{2.417}
\expandafter\def\csname R@oneill/abl/t/repl/6/none\endcsname{2.398}
\expandafter\def\csname R@oneill/abl/t/repl/6/repeat\endcsname{2.424}
\expandafter\def\csname R@oneill/abl/t/repl/96\endcsname{1.491}
\expandafter\def\csname R@oneill/abl/t/repl/96/none\endcsname{1.648}
\expandafter\def\csname R@oneill/abl/t/repl/96/repeat\endcsname{1.434}
\expandafter\def\csname R@oneill/abl/t/sweep/18\endcsname{1.543}
\expandafter\def\csname R@oneill/abl/t/sweep/192\endcsname{0.791}
\expandafter\def\csname R@oneill/abl/t/sweep/336\endcsname{0.497}
\expandafter\def\csname R@oneill/abl/t/sweep/48\endcsname{1.449}
\expandafter\def\csname R@oneill/abl/t/sweep/6\endcsname{1.692}
\expandafter\def\csname R@oneill/abl/t/sweep/96\endcsname{1.160}
\expandafter\def\csname R@oneill/abl/t/trunc/18\endcsname{2.462}
\expandafter\def\csname R@oneill/abl/t/trunc/18/none\endcsname{2.459}
\expandafter\def\csname R@oneill/abl/t/trunc/18/repeat\endcsname{2.463}
\expandafter\def\csname R@oneill/abl/t/trunc/192\endcsname{0.861}
\expandafter\def\csname R@oneill/abl/t/trunc/192/none\endcsname{1.326}
\expandafter\def\csname R@oneill/abl/t/trunc/192/repeat\endcsname{0.692}
\expandafter\def\csname R@oneill/abl/t/trunc/336\endcsname{0.497}
\expandafter\def\csname R@oneill/abl/t/trunc/336/none\endcsname{1.245}
\expandafter\def\csname R@oneill/abl/t/trunc/336/repeat\endcsname{0.223}
\expandafter\def\csname R@oneill/abl/t/trunc/48\endcsname{1.981}
\expandafter\def\csname R@oneill/abl/t/trunc/48/none\endcsname{2.016}
\expandafter\def\csname R@oneill/abl/t/trunc/48/repeat\endcsname{1.969}
\expandafter\def\csname R@oneill/abl/t/trunc/6\endcsname{3.381}
\expandafter\def\csname R@oneill/abl/t/trunc/6/none\endcsname{3.442}
\expandafter\def\csname R@oneill/abl/t/trunc/6/repeat\endcsname{3.359}
\expandafter\def\csname R@oneill/abl/t/trunc/96\endcsname{1.460}
\expandafter\def\csname R@oneill/abl/t/trunc/96/none\endcsname{1.610}
\expandafter\def\csname R@oneill/abl/t/trunc/96/repeat\endcsname{1.406}
\expandafter\def\csname R@oneill/abl/targets\endcsname{72{,}240}
\expandafter\def\csname R@oneill/ae/acc\endcsname{99.993}
\expandafter\def\csname R@oneill/align/192/aligned\endcsname{0.15}
\expandafter\def\csname R@oneill/align/192/misaligned\endcsname{0.82}
\expandafter\def\csname R@oneill/align/192/share\endcsname{67}
\expandafter\def\csname R@oneill/align/336/aligned\endcsname{0.10}
\expandafter\def\csname R@oneill/align/336/misaligned\endcsname{0.76}
\expandafter\def\csname R@oneill/align/336/share\endcsname{72}
\expandafter\def\csname R@oneill/align/96/aligned\endcsname{0.42}
\expandafter\def\csname R@oneill/align/96/misaligned\endcsname{0.86}
\expandafter\def\csname R@oneill/align/96/share\endcsname{75}
\expandafter\def\csname R@oneill/aligned/1-32\endcsname{54}
\expandafter\def\csname R@oneill/aligned/177-320\endcsname{79}
\expandafter\def\csname R@oneill/aligned/33-80\endcsname{82}
\expandafter\def\csname R@oneill/aligned/81-176\endcsname{67}
\expandafter\def\csname R@oneill/aligned/all\endcsname{74}
\expandafter\def\csname R@oneill/boot/l/18-48\endcsname{0.046}
\expandafter\def\csname R@oneill/boot/l/18-48/hi\endcsname{0.051}
\expandafter\def\csname R@oneill/boot/l/18-48/lo\endcsname{0.039}
\expandafter\def\csname R@oneill/boot/l/18-6\endcsname{-0.028}
\expandafter\def\csname R@oneill/boot/l/18-6/hi\endcsname{-0.018}
\expandafter\def\csname R@oneill/boot/l/18-6/lo\endcsname{-0.042}
\expandafter\def\csname R@oneill/boot/l/192-336\endcsname{0.161}
\expandafter\def\csname R@oneill/boot/l/192-336/hi\endcsname{0.215}
\expandafter\def\csname R@oneill/boot/l/192-336/lo\endcsname{0.092}
\expandafter\def\csname R@oneill/boot/l/192-96\endcsname{-0.150}
\expandafter\def\csname R@oneill/boot/l/192-96/hi\endcsname{-0.106}
\expandafter\def\csname R@oneill/boot/l/192-96/lo\endcsname{-0.181}
\expandafter\def\csname R@oneill/boot/l/336-192\endcsname{-0.161}
\expandafter\def\csname R@oneill/boot/l/336-192/hi\endcsname{-0.092}
\expandafter\def\csname R@oneill/boot/l/336-192/lo\endcsname{-0.215}
\expandafter\def\csname R@oneill/boot/l/336-48\endcsname{-0.353}
\expandafter\def\csname R@oneill/boot/l/336-48/hi\endcsname{-0.235}
\expandafter\def\csname R@oneill/boot/l/336-48/lo\endcsname{-0.437}
\expandafter\def\csname R@oneill/boot/l/336-6\endcsname{-0.427}
\expandafter\def\csname R@oneill/boot/l/336-6/hi\endcsname{-0.300}
\expandafter\def\csname R@oneill/boot/l/336-6/lo\endcsname{-0.523}
\expandafter\def\csname R@oneill/boot/l/336-96\endcsname{-0.312}
\expandafter\def\csname R@oneill/boot/l/336-96/hi\endcsname{-0.203}
\expandafter\def\csname R@oneill/boot/l/336-96/lo\endcsname{-0.382}
\expandafter\def\csname R@oneill/boot/l/48-18\endcsname{-0.046}
\expandafter\def\csname R@oneill/boot/l/48-18/hi\endcsname{-0.039}
\expandafter\def\csname R@oneill/boot/l/48-18/lo\endcsname{-0.051}
\expandafter\def\csname R@oneill/boot/l/48-336\endcsname{0.353}
\expandafter\def\csname R@oneill/boot/l/48-336/hi\endcsname{0.437}
\expandafter\def\csname R@oneill/boot/l/48-336/lo\endcsname{0.235}
\expandafter\def\csname R@oneill/boot/l/48-96\endcsname{0.041}
\expandafter\def\csname R@oneill/boot/l/48-96/hi\endcsname{0.066}
\expandafter\def\csname R@oneill/boot/l/48-96/lo\endcsname{0.029}
\expandafter\def\csname R@oneill/boot/l/6-18\endcsname{0.028}
\expandafter\def\csname R@oneill/boot/l/6-18/hi\endcsname{0.042}
\expandafter\def\csname R@oneill/boot/l/6-18/lo\endcsname{0.018}
\expandafter\def\csname R@oneill/boot/l/6-336\endcsname{0.427}
\expandafter\def\csname R@oneill/boot/l/6-336/hi\endcsname{0.523}
\expandafter\def\csname R@oneill/boot/l/6-336/lo\endcsname{0.300}
\expandafter\def\csname R@oneill/boot/l/96-192\endcsname{0.150}
\expandafter\def\csname R@oneill/boot/l/96-192/hi\endcsname{0.181}
\expandafter\def\csname R@oneill/boot/l/96-192/lo\endcsname{0.106}
\expandafter\def\csname R@oneill/boot/l/96-336\endcsname{0.312}
\expandafter\def\csname R@oneill/boot/l/96-336/hi\endcsname{0.382}
\expandafter\def\csname R@oneill/boot/l/96-336/lo\endcsname{0.203}
\expandafter\def\csname R@oneill/boot/l/96-48\endcsname{-0.041}
\expandafter\def\csname R@oneill/boot/l/96-48/hi\endcsname{-0.029}
\expandafter\def\csname R@oneill/boot/l/96-48/lo\endcsname{-0.066}
\expandafter\def\csname R@oneill/boot/t/18-48\endcsname{0.094}
\expandafter\def\csname R@oneill/boot/t/18-48/hi\endcsname{0.149}
\expandafter\def\csname R@oneill/boot/t/18-48/lo\endcsname{0.051}
\expandafter\def\csname R@oneill/boot/t/18-6\endcsname{-0.149}
\expandafter\def\csname R@oneill/boot/t/18-6/hi\endcsname{-0.122}
\expandafter\def\csname R@oneill/boot/t/18-6/lo\endcsname{-0.197}
\expandafter\def\csname R@oneill/boot/t/192-336\endcsname{0.294}
\expandafter\def\csname R@oneill/boot/t/192-336/hi\endcsname{0.329}
\expandafter\def\csname R@oneill/boot/t/192-336/lo\endcsname{0.265}
\expandafter\def\csname R@oneill/boot/t/192-96\endcsname{-0.369}
\expandafter\def\csname R@oneill/boot/t/192-96/hi\endcsname{-0.335}
\expandafter\def\csname R@oneill/boot/t/192-96/lo\endcsname{-0.455}
\expandafter\def\csname R@oneill/boot/t/336-192\endcsname{-0.294}
\expandafter\def\csname R@oneill/boot/t/336-192/hi\endcsname{-0.265}
\expandafter\def\csname R@oneill/boot/t/336-192/lo\endcsname{-0.329}
\expandafter\def\csname R@oneill/boot/t/336-48\endcsname{-0.953}
\expandafter\def\csname R@oneill/boot/t/336-48/hi\endcsname{-0.898}
\expandafter\def\csname R@oneill/boot/t/336-48/lo\endcsname{-1.091}
\expandafter\def\csname R@oneill/boot/t/336-6\endcsname{-1.195}
\expandafter\def\csname R@oneill/boot/t/336-6/hi\endcsname{-1.105}
\expandafter\def\csname R@oneill/boot/t/336-6/lo\endcsname{-1.385}
\expandafter\def\csname R@oneill/boot/t/336-96\endcsname{-0.663}
\expandafter\def\csname R@oneill/boot/t/336-96/hi\endcsname{-0.612}
\expandafter\def\csname R@oneill/boot/t/336-96/lo\endcsname{-0.770}
\expandafter\def\csname R@oneill/boot/t/48-18\endcsname{-0.094}
\expandafter\def\csname R@oneill/boot/t/48-18/hi\endcsname{-0.051}
\expandafter\def\csname R@oneill/boot/t/48-18/lo\endcsname{-0.149}
\expandafter\def\csname R@oneill/boot/t/48-336\endcsname{0.953}
\expandafter\def\csname R@oneill/boot/t/48-336/hi\endcsname{1.091}
\expandafter\def\csname R@oneill/boot/t/48-336/lo\endcsname{0.898}
\expandafter\def\csname R@oneill/boot/t/48-96\endcsname{0.290}
\expandafter\def\csname R@oneill/boot/t/48-96/hi\endcsname{0.366}
\expandafter\def\csname R@oneill/boot/t/48-96/lo\endcsname{0.227}
\expandafter\def\csname R@oneill/boot/t/6-18\endcsname{0.149}
\expandafter\def\csname R@oneill/boot/t/6-18/hi\endcsname{0.197}
\expandafter\def\csname R@oneill/boot/t/6-18/lo\endcsname{0.122}
\expandafter\def\csname R@oneill/boot/t/6-336\endcsname{1.195}
\expandafter\def\csname R@oneill/boot/t/6-336/hi\endcsname{1.385}
\expandafter\def\csname R@oneill/boot/t/6-336/lo\endcsname{1.105}
\expandafter\def\csname R@oneill/boot/t/96-192\endcsname{0.369}
\expandafter\def\csname R@oneill/boot/t/96-192/hi\endcsname{0.455}
\expandafter\def\csname R@oneill/boot/t/96-192/lo\endcsname{0.335}
\expandafter\def\csname R@oneill/boot/t/96-336\endcsname{0.663}
\expandafter\def\csname R@oneill/boot/t/96-336/hi\endcsname{0.770}
\expandafter\def\csname R@oneill/boot/t/96-336/lo\endcsname{0.612}
\expandafter\def\csname R@oneill/boot/t/96-48\endcsname{-0.290}
\expandafter\def\csname R@oneill/boot/t/96-48/hi\endcsname{-0.227}
\expandafter\def\csname R@oneill/boot/t/96-48/lo\endcsname{-0.366}
\expandafter\def\csname R@oneill/clamped\endcsname{0.0}
\expandafter\def\csname R@oneill/copy/s/1-32\endcsname{12}
\expandafter\def\csname R@oneill/copy/s/177-320\endcsname{95}
\expandafter\def\csname R@oneill/copy/s/33-80\endcsname{53}
\expandafter\def\csname R@oneill/copy/s/81-176\endcsname{88}
\expandafter\def\csname R@oneill/copy/s/all\endcsname{85}
\expandafter\def\csname R@oneill/copy/t/1-32\endcsname{62}
\expandafter\def\csname R@oneill/copy/t/177-320\endcsname{99}
\expandafter\def\csname R@oneill/copy/t/33-80\endcsname{90}
\expandafter\def\csname R@oneill/copy/t/81-176\endcsname{98}
\expandafter\def\csname R@oneill/copy/t/all\endcsname{97}
\expandafter\def\csname R@oneill/copybase/16\endcsname{0.644}
\expandafter\def\csname R@oneill/copybase/16/gain\endcsname{88}
\expandafter\def\csname R@oneill/copybase/16/matched\endcsname{73}
\expandafter\def\csname R@oneill/copybase/backoff\endcsname{0.533}
\expandafter\def\csname R@oneill/copybase/backoff/gain\endcsname{97}
\expandafter\def\csname R@oneill/copybase/backoff/matched\endcsname{81}
\expandafter\def\csname R@oneill/copybase/base\endcsname{1.692}
\expandafter\def\csname R@oneill/copybase/m/bits_T336\endcsname{0.29}
\expandafter\def\csname R@oneill/copybase/m/bits_T6\endcsname{1.70}
\expandafter\def\csname R@oneill/copybase/m/bits_copy\endcsname{0.27}
\expandafter\def\csname R@oneill/copybase/m/copy\endcsname{97}
\expandafter\def\csname R@oneill/copybase/m/t336\endcsname{95}
\expandafter\def\csname R@oneill/groups\endcsname{1828}
\expandafter\def\csname R@oneill/h32/copy\endcsname{99}
\expandafter\def\csname R@oneill/h32/redshare/l\endcsname{82}
\expandafter\def\csname R@oneill/h32/redshare/t\endcsname{79}
\expandafter\def\csname R@oneill/h32/share\endcsname{64}
\expandafter\def\csname R@oneill/h8/copy\endcsname{93}
\expandafter\def\csname R@oneill/h8/redshare/l\endcsname{95}
\expandafter\def\csname R@oneill/h8/redshare/t\endcsname{94}
\expandafter\def\csname R@oneill/h8/share\endcsname{80}
\expandafter\def\csname R@oneill/inview/18\endcsname{0.0}
\expandafter\def\csname R@oneill/inview/192\endcsname{43.2}
\expandafter\def\csname R@oneill/inview/336\endcsname{73.3}
\expandafter\def\csname R@oneill/inview/48\endcsname{0.3}
\expandafter\def\csname R@oneill/inview/6\endcsname{0.0}
\expandafter\def\csname R@oneill/inview/96\endcsname{9.9}
\expandafter\def\csname R@oneill/lag/l/18/1-32\endcsname{0.85}
\expandafter\def\csname R@oneill/lag/l/18/177-320\endcsname{0.82}
\expandafter\def\csname R@oneill/lag/l/18/33-80\endcsname{0.81}
\expandafter\def\csname R@oneill/lag/l/18/81-176\endcsname{0.83}
\expandafter\def\csname R@oneill/lag/l/18/held\endcsname{0.77}
\expandafter\def\csname R@oneill/lag/l/18/none\endcsname{0.81}
\expandafter\def\csname R@oneill/lag/l/192/1-32\endcsname{0.64}
\expandafter\def\csname R@oneill/lag/l/192/177-320\endcsname{0.66}
\expandafter\def\csname R@oneill/lag/l/192/33-80\endcsname{0.47}
\expandafter\def\csname R@oneill/lag/l/192/81-176\endcsname{0.46}
\expandafter\def\csname R@oneill/lag/l/192/held\endcsname{0.63}
\expandafter\def\csname R@oneill/lag/l/192/none\endcsname{0.69}
\expandafter\def\csname R@oneill/lag/l/336/1-32\endcsname{0.51}
\expandafter\def\csname R@oneill/lag/l/336/177-320\endcsname{0.26}
\expandafter\def\csname R@oneill/lag/l/336/33-80\endcsname{0.30}
\expandafter\def\csname R@oneill/lag/l/336/81-176\endcsname{0.40}
\expandafter\def\csname R@oneill/lag/l/336/held\endcsname{0.10}
\expandafter\def\csname R@oneill/lag/l/336/none\endcsname{0.68}
\expandafter\def\csname R@oneill/lag/l/48/1-32\endcsname{0.74}
\expandafter\def\csname R@oneill/lag/l/48/177-320\endcsname{0.77}
\expandafter\def\csname R@oneill/lag/l/48/33-80\endcsname{0.75}
\expandafter\def\csname R@oneill/lag/l/48/81-176\endcsname{0.78}
\expandafter\def\csname R@oneill/lag/l/48/held\endcsname{0.76}
\expandafter\def\csname R@oneill/lag/l/48/none\endcsname{0.78}
\expandafter\def\csname R@oneill/lag/l/6/1-32\endcsname{0.91}
\expandafter\def\csname R@oneill/lag/l/6/177-320\endcsname{0.84}
\expandafter\def\csname R@oneill/lag/l/6/33-80\endcsname{0.85}
\expandafter\def\csname R@oneill/lag/l/6/81-176\endcsname{0.85}
\expandafter\def\csname R@oneill/lag/l/6/held\endcsname{0.81}
\expandafter\def\csname R@oneill/lag/l/6/none\endcsname{0.83}
\expandafter\def\csname R@oneill/lag/l/96/1-32\endcsname{0.74}
\expandafter\def\csname R@oneill/lag/l/96/177-320\endcsname{0.73}
\expandafter\def\csname R@oneill/lag/l/96/33-80\endcsname{0.68}
\expandafter\def\csname R@oneill/lag/l/96/81-176\endcsname{0.73}
\expandafter\def\csname R@oneill/lag/l/96/held\endcsname{0.59}
\expandafter\def\csname R@oneill/lag/l/96/none\endcsname{0.75}
\expandafter\def\csname R@oneill/lag/t/18/1-32\endcsname{2.31}
\expandafter\def\csname R@oneill/lag/t/18/177-320\endcsname{1.52}
\expandafter\def\csname R@oneill/lag/t/18/33-80\endcsname{1.59}
\expandafter\def\csname R@oneill/lag/t/18/81-176\endcsname{1.51}
\expandafter\def\csname R@oneill/lag/t/18/held\endcsname{1.14}
\expandafter\def\csname R@oneill/lag/t/18/none\endcsname{1.59}
\expandafter\def\csname R@oneill/lag/t/192/1-32\endcsname{0.96}
\expandafter\def\csname R@oneill/lag/t/192/177-320\endcsname{1.05}
\expandafter\def\csname R@oneill/lag/t/192/33-80\endcsname{0.44}
\expandafter\def\csname R@oneill/lag/t/192/81-176\endcsname{0.35}
\expandafter\def\csname R@oneill/lag/t/192/held\endcsname{0.23}
\expandafter\def\csname R@oneill/lag/t/192/none\endcsname{1.17}
\expandafter\def\csname R@oneill/lag/t/336/1-32\endcsname{0.64}
\expandafter\def\csname R@oneill/lag/t/336/177-320\endcsname{0.20}
\expandafter\def\csname R@oneill/lag/t/336/33-80\endcsname{0.26}
\expandafter\def\csname R@oneill/lag/t/336/81-176\endcsname{0.23}
\expandafter\def\csname R@oneill/lag/t/336/held\endcsname{0.09}
\expandafter\def\csname R@oneill/lag/t/336/none\endcsname{1.25}
\expandafter\def\csname R@oneill/lag/t/48/1-32\endcsname{2.25}
\expandafter\def\csname R@oneill/lag/t/48/177-320\endcsname{1.42}
\expandafter\def\csname R@oneill/lag/t/48/33-80\endcsname{1.51}
\expandafter\def\csname R@oneill/lag/t/48/81-176\endcsname{1.43}
\expandafter\def\csname R@oneill/lag/t/48/held\endcsname{0.36}
\expandafter\def\csname R@oneill/lag/t/48/none\endcsname{1.48}
\expandafter\def\csname R@oneill/lag/t/6/1-32\endcsname{2.49}
\expandafter\def\csname R@oneill/lag/t/6/177-320\endcsname{1.64}
\expandafter\def\csname R@oneill/lag/t/6/33-80\endcsname{1.79}
\expandafter\def\csname R@oneill/lag/t/6/81-176\endcsname{1.70}
\expandafter\def\csname R@oneill/lag/t/6/held\endcsname{0.95}
\expandafter\def\csname R@oneill/lag/t/6/none\endcsname{1.70}
\expandafter\def\csname R@oneill/lag/t/96/1-32\endcsname{1.36}
\expandafter\def\csname R@oneill/lag/t/96/177-320\endcsname{1.15}
\expandafter\def\csname R@oneill/lag/t/96/33-80\endcsname{0.80}
\expandafter\def\csname R@oneill/lag/t/96/81-176\endcsname{1.16}
\expandafter\def\csname R@oneill/lag/t/96/held\endcsname{0.34}
\expandafter\def\csname R@oneill/lag/t/96/none\endcsname{1.30}
\expandafter\def\csname R@oneill/lat/0\endcsname{0.931}
\expandafter\def\csname R@oneill/lat/0/n\endcsname{1}
\expandafter\def\csname R@oneill/lat/0/pertoken\endcsname{9.93}
\expandafter\def\csname R@oneill/lat/18\endcsname{0.818}
\expandafter\def\csname R@oneill/lat/18/ep/max\endcsname{87}
\expandafter\def\csname R@oneill/lat/18/ep/min\endcsname{48}
\expandafter\def\csname R@oneill/lat/18/n\endcsname{3}
\expandafter\def\csname R@oneill/lat/18/pertoken\endcsname{8.72}
\expandafter\def\csname R@oneill/lat/18/sd\endcsname{0.003}
\expandafter\def\csname R@oneill/lat/192\endcsname{0.580}
\expandafter\def\csname R@oneill/lat/192/ep/max\endcsname{123}
\expandafter\def\csname R@oneill/lat/192/ep/min\endcsname{97}
\expandafter\def\csname R@oneill/lat/192/n\endcsname{3}
\expandafter\def\csname R@oneill/lat/192/pertoken\endcsname{6.19}
\expandafter\def\csname R@oneill/lat/192/sd\endcsname{0.002}
\expandafter\def\csname R@oneill/lat/336\endcsname{0.419}
\expandafter\def\csname R@oneill/lat/336/ep/max\endcsname{119}
\expandafter\def\csname R@oneill/lat/336/ep/min\endcsname{89}
\expandafter\def\csname R@oneill/lat/336/n\endcsname{3}
\expandafter\def\csname R@oneill/lat/336/pertoken\endcsname{4.46}
\expandafter\def\csname R@oneill/lat/336/sd\endcsname{0.007}
\expandafter\def\csname R@oneill/lat/48\endcsname{0.771}
\expandafter\def\csname R@oneill/lat/48/ep/max\endcsname{121}
\expandafter\def\csname R@oneill/lat/48/ep/min\endcsname{68}
\expandafter\def\csname R@oneill/lat/48/n\endcsname{3}
\expandafter\def\csname R@oneill/lat/48/pertoken\endcsname{8.23}
\expandafter\def\csname R@oneill/lat/48/sd\endcsname{0.005}
\expandafter\def\csname R@oneill/lat/6\endcsname{0.845}
\expandafter\def\csname R@oneill/lat/6/ep/max\endcsname{5}
\expandafter\def\csname R@oneill/lat/6/ep/min\endcsname{2}
\expandafter\def\csname R@oneill/lat/6/n\endcsname{3}
\expandafter\def\csname R@oneill/lat/6/pertoken\endcsname{9.02}
\expandafter\def\csname R@oneill/lat/6/sd\endcsname{0.005}
\expandafter\def\csname R@oneill/lat/96\endcsname{0.730}
\expandafter\def\csname R@oneill/lat/96/ep/max\endcsname{139}
\expandafter\def\csname R@oneill/lat/96/ep/min\endcsname{79}
\expandafter\def\csname R@oneill/lat/96/n\endcsname{3}
\expandafter\def\csname R@oneill/lat/96/pertoken\endcsname{7.79}
\expandafter\def\csname R@oneill/lat/96/sd\endcsname{0.009}
\expandafter\def\csname R@oneill/lat/drop\endcsname{50}
\expandafter\def\csname R@oneill/lat/ep/max\endcsname{139}
\expandafter\def\csname R@oneill/lat/maxsd\endcsname{0.009}
\expandafter\def\csname R@oneill/leak/test/verbatim\endcsname{0.6}
\expandafter\def\csname R@oneill/long/test\endcsname{129}
\expandafter\def\csname R@oneill/long/train\endcsname{601}
\expandafter\def\csname R@oneill/longep/max\endcsname{123}
\expandafter\def\csname R@oneill/longep/min\endcsname{35}
\expandafter\def\csname R@oneill/merged\endcsname{166}
\expandafter\def\csname R@oneill/moved\endcsname{0}
\expandafter\def\csname R@oneill/ov/blocks\endcsname{3195}
\expandafter\def\csname R@oneill/ov/drop/all\endcsname{70.6}
\expandafter\def\csname R@oneill/ov/drop/without\endcsname{70.3}
\expandafter\def\csname R@oneill/ov/max\endcsname{49}
\expandafter\def\csname R@oneill/ov/min\endcsname{30}
\expandafter\def\csname R@oneill/ov/tunes\endcsname{7}
\expandafter\def\csname R@oneill/ov/verbatim\endcsname{18}
\expandafter\def\csname R@oneill/pieces/all\endcsname{1994}
\expandafter\def\csname R@oneill/pieces/test\endcsname{302}
\expandafter\def\csname R@oneill/pieces/testwin\endcsname{129}
\expandafter\def\csname R@oneill/pieces/train\endcsname{1397}
\expandafter\def\csname R@oneill/pieces/val\endcsname{295}
\expandafter\def\csname R@oneill/pitchlo\endcsname{42}
\expandafter\def\csname R@oneill/reached/l/18\endcsname{7}
\expandafter\def\csname R@oneill/reached/l/192\endcsname{62}
\expandafter\def\csname R@oneill/reached/l/336\endcsname{100}
\expandafter\def\csname R@oneill/reached/l/48\endcsname{17}
\expandafter\def\csname R@oneill/reached/l/6\endcsname{0}
\expandafter\def\csname R@oneill/reached/l/96\endcsname{27}
\expandafter\def\csname R@oneill/reached/t/18\endcsname{12}
\expandafter\def\csname R@oneill/reached/t/192\endcsname{75}
\expandafter\def\csname R@oneill/reached/t/336\endcsname{100}
\expandafter\def\csname R@oneill/reached/t/48\endcsname{20}
\expandafter\def\csname R@oneill/reached/t/6\endcsname{0}
\expandafter\def\csname R@oneill/reached/t/96\endcsname{45}
\expandafter\def\csname R@oneill/redshare/l/none\endcsname{9}
\expandafter\def\csname R@oneill/redshare/l/repeat\endcsname{91}
\expandafter\def\csname R@oneill/redshare/t/none\endcsname{10}
\expandafter\def\csname R@oneill/redshare/t/repeat\endcsname{90}
\expandafter\def\csname R@oneill/rest\endcsname{0.3}
\expandafter\def\csname R@oneill/sel/dropped/median\endcsname{256}
\expandafter\def\csname R@oneill/sel/dropped/n\endcsname{173}
\expandafter\def\csname R@oneill/sel/dropped/repeat\endcsname{24}
\expandafter\def\csname R@oneill/sel/dropped/repeat256\endcsname{23}
\expandafter\def\csname R@oneill/sel/kept/median\endcsname{576}
\expandafter\def\csname R@oneill/sel/kept/n\endcsname{129}
\expandafter\def\csname R@oneill/sel/kept/repeat\endcsname{63}
\expandafter\def\csname R@oneill/sel/kept/repeat256\endcsname{43}
\expandafter\def\csname R@oneill/share/s/1-32\endcsname{0.4}
\expandafter\def\csname R@oneill/share/s/177-320\endcsname{29.1}
\expandafter\def\csname R@oneill/share/s/33-80\endcsname{11.1}
\expandafter\def\csname R@oneill/share/s/81-176\endcsname{33.8}
\expandafter\def\csname R@oneill/share/s/held\endcsname{0.0}
\expandafter\def\csname R@oneill/share/s/none\endcsname{25.6}
\expandafter\def\csname R@oneill/share/s/repeat\endcsname{74}
\expandafter\def\csname R@oneill/share/t/1-32\endcsname{0.3}
\expandafter\def\csname R@oneill/share/t/177-320\endcsname{30.1}
\expandafter\def\csname R@oneill/share/t/33-80\endcsname{9.6}
\expandafter\def\csname R@oneill/share/t/81-176\endcsname{33.3}
\expandafter\def\csname R@oneill/share/t/held\endcsname{0.0}
\expandafter\def\csname R@oneill/share/t/none\endcsname{26.7}
\expandafter\def\csname R@oneill/share/t/repeat\endcsname{73}
\expandafter\def\csname R@oneill/targets\endcsname{48}
\expandafter\def\csname R@oneill/tok/0\endcsname{4.383}
\expandafter\def\csname R@oneill/tok/0/n\endcsname{1}
\expandafter\def\csname R@oneill/tok/18\endcsname{1.543}
\expandafter\def\csname R@oneill/tok/18/ep/max\endcsname{201}
\expandafter\def\csname R@oneill/tok/18/ep/min\endcsname{78}
\expandafter\def\csname R@oneill/tok/18/n\endcsname{3}
\expandafter\def\csname R@oneill/tok/18/sd\endcsname{0.019}
\expandafter\def\csname R@oneill/tok/192\endcsname{0.791}
\expandafter\def\csname R@oneill/tok/192/ep/max\endcsname{99}
\expandafter\def\csname R@oneill/tok/192/ep/min\endcsname{74}
\expandafter\def\csname R@oneill/tok/192/n\endcsname{3}
\expandafter\def\csname R@oneill/tok/192/sd\endcsname{0.012}
\expandafter\def\csname R@oneill/tok/336\endcsname{0.497}
\expandafter\def\csname R@oneill/tok/336/ep/max\endcsname{102}
\expandafter\def\csname R@oneill/tok/336/ep/min\endcsname{35}
\expandafter\def\csname R@oneill/tok/336/n\endcsname{3}
\expandafter\def\csname R@oneill/tok/336/sd\endcsname{0.011}
\expandafter\def\csname R@oneill/tok/48\endcsname{1.449}
\expandafter\def\csname R@oneill/tok/48/ep/max\endcsname{135}
\expandafter\def\csname R@oneill/tok/48/ep/min\endcsname{109}
\expandafter\def\csname R@oneill/tok/48/n\endcsname{3}
\expandafter\def\csname R@oneill/tok/48/sd\endcsname{0.017}
\expandafter\def\csname R@oneill/tok/6\endcsname{1.692}
\expandafter\def\csname R@oneill/tok/6/ep/max\endcsname{31}
\expandafter\def\csname R@oneill/tok/6/ep/min\endcsname{12}
\expandafter\def\csname R@oneill/tok/6/n\endcsname{3}
\expandafter\def\csname R@oneill/tok/6/sd\endcsname{0.014}
\expandafter\def\csname R@oneill/tok/96\endcsname{1.160}
\expandafter\def\csname R@oneill/tok/96/ep/max\endcsname{157}
\expandafter\def\csname R@oneill/tok/96/ep/min\endcsname{95}
\expandafter\def\csname R@oneill/tok/96/n\endcsname{3}
\expandafter\def\csname R@oneill/tok/96/sd\endcsname{0.015}
\expandafter\def\csname R@oneill/tok/drop\endcsname{71}
\expandafter\def\csname R@oneill/tok/ep/max\endcsname{201}
\expandafter\def\csname R@oneill/tok/maxsd\endcsname{0.019}
\expandafter\def\csname R@oneill/tokens/test\endcsname{158{,}043}
\expandafter\def\csname R@oneill/tokens/train\endcsname{738{,}428}
\expandafter\def\csname R@oneill/tokens/val\endcsname{115{,}286}
\expandafter\def\csname R@oneill/trans/copy\endcsname{78}
\expandafter\def\csname R@oneill/trans/other/336\endcsname{1.25}
\expandafter\def\csname R@oneill/trans/other/6\endcsname{1.69}
\expandafter\def\csname R@oneill/trans/share\endcsname{0.0}
\expandafter\def\csname R@oneill/trans/t/336\endcsname{2.31}
\expandafter\def\csname R@oneill/trans/t/6\endcsname{3.09}
\expandafter\def\csname R@oneill/unusable\endcsname{15}
\expandafter\def\csname R@oneill/v5/0\endcsname{0.931}
\expandafter\def\csname R@oneill/v5/0/n\endcsname{1}
\expandafter\def\csname R@oneill/win/test\endcsname{1505}
\expandafter\def\csname R@oneill/win/train\endcsname{7121}
\expandafter\def\csname R@oneill/window\endcsname{384}
\expandafter\def\csname R@params/lat\endcsname{2.49M}
\expandafter\def\csname R@params/tok\endcsname{2.50M}
\expandafter\def\csname R@params/tok89\endcsname{2.53M}
\expandafter\def\csname R@params/v5\endcsname{2.31M}
\expandafter\def\csname R@seeds/192/above6\endcsname{0}
\expandafter\def\csname R@seeds/192/best/max\endcsname{200}
\expandafter\def\csname R@seeds/192/best/min\endcsname{162}
\expandafter\def\csname R@seeds/192/drop/max\endcsname{60}
\expandafter\def\csname R@seeds/192/drop/min\endcsname{34}
\expandafter\def\csname R@seeds/192/drop/n\endcsname{10}
\expandafter\def\csname R@seeds/192/drop/nll/max\endcsname{0.56}
\expandafter\def\csname R@seeds/192/drop/nll/min\endcsname{0.55}
\expandafter\def\csname R@seeds/192/drop/nll/second\endcsname{0.56}
\expandafter\def\csname R@seeds/192/escut\endcsname{0}
\expandafter\def\csname R@seeds/192/inview/max\endcsname{0.23}
\expandafter\def\csname R@seeds/192/inview/min\endcsname{0.22}
\expandafter\def\csname R@seeds/192/max\endcsname{0.56}
\expandafter\def\csname R@seeds/192/min\endcsname{0.55}
\expandafter\def\csname R@seeds/192/n\endcsname{10}
\expandafter\def\csname R@seeds/48/above6\endcsname{10}
\expandafter\def\csname R@seeds/48/best/max\endcsname{200}
\expandafter\def\csname R@seeds/48/best/min\endcsname{41}
\expandafter\def\csname R@seeds/48/drop/max\endcsname{44}
\expandafter\def\csname R@seeds/48/drop/min\endcsname{44}
\expandafter\def\csname R@seeds/48/drop/n\endcsname{1}
\expandafter\def\csname R@seeds/48/drop/nll/max\endcsname{1.49}
\expandafter\def\csname R@seeds/48/drop/nll/min\endcsname{1.49}
\expandafter\def\csname R@seeds/48/drop/nll/second\endcsname{1.49}
\expandafter\def\csname R@seeds/48/escut\endcsname{0}
\expandafter\def\csname R@seeds/48/inview/max\endcsname{2.10}
\expandafter\def\csname R@seeds/48/inview/min\endcsname{1.80}
\expandafter\def\csname R@seeds/48/max\endcsname{1.61}
\expandafter\def\csname R@seeds/48/min\endcsname{1.49}
\expandafter\def\csname R@seeds/48/n\endcsname{10}
\expandafter\def\csname R@seeds/48/nodrop/es/max\endcsname{74}
\expandafter\def\csname R@seeds/48/nodrop/es/min\endcsname{55}
\expandafter\def\csname R@seeds/48/nodrop/inview/max\endcsname{2.10}
\expandafter\def\csname R@seeds/48/nodrop/inview/min\endcsname{1.80}
\expandafter\def\csname R@seeds/48/nodrop/nll/max\endcsname{1.61}
\expandafter\def\csname R@seeds/48/nodrop/nll/min\endcsname{1.49}
\expandafter\def\csname R@seeds/48/nodrop/none/max\endcsname{1.55}
\expandafter\def\csname R@seeds/48/nodrop/none/min\endcsname{1.43}
\expandafter\def\csname R@seeds/96/above6\endcsname{1}
\expandafter\def\csname R@seeds/96/best/max\endcsname{193}
\expandafter\def\csname R@seeds/96/best/min\endcsname{135}
\expandafter\def\csname R@seeds/96/drop/max\endcsname{172}
\expandafter\def\csname R@seeds/96/drop/min\endcsname{41}
\expandafter\def\csname R@seeds/96/drop/n\endcsname{6}
\expandafter\def\csname R@seeds/96/drop/nll/max\endcsname{1.26}
\expandafter\def\csname R@seeds/96/drop/nll/min\endcsname{0.89}
\expandafter\def\csname R@seeds/96/drop/nll/second\endcsname{0.99}
\expandafter\def\csname R@seeds/96/escut\endcsname{2}
\expandafter\def\csname R@seeds/96/inview/max\endcsname{1.00}
\expandafter\def\csname R@seeds/96/inview/min\endcsname{0.52}
\expandafter\def\csname R@seeds/96/max\endcsname{1.40}
\expandafter\def\csname R@seeds/96/min\endcsname{0.89}
\expandafter\def\csname R@seeds/96/n\endcsname{10}
\expandafter\def\csname R@seeds/96/nodrop/es/max\endcsname{192}
\expandafter\def\csname R@seeds/96/nodrop/es/min\endcsname{49}
\expandafter\def\csname R@seeds/96/nodrop/inview/max\endcsname{1.00}
\expandafter\def\csname R@seeds/96/nodrop/inview/min\endcsname{0.96}
\expandafter\def\csname R@seeds/96/nodrop/nll/max\endcsname{1.40}
\expandafter\def\csname R@seeds/96/nodrop/nll/min\endcsname{1.34}
\expandafter\def\csname R@seeds/96/nodrop/none/max\endcsname{1.49}
\expandafter\def\csname R@seeds/96/nodrop/none/min\endcsname{1.41}
\expandafter\def\csname R@sweepdrop/long/max\endcsname{49}
\expandafter\def\csname R@sweepdrop/long/min\endcsname{31}
\expandafter\def\csname R@sweepseed/192/s0/inview\endcsname{0.23}
\expandafter\def\csname R@sweepseed/192/s0/none\endcsname{0.94}
\expandafter\def\csname R@sweepseed/192/s0/stop\endcsname{145}
\expandafter\def\csname R@sweepseed/192/s0/test\endcsname{0.57}
\expandafter\def\csname R@sweepseed/192/s42/inview\endcsname{0.23}
\expandafter\def\csname R@sweepseed/192/s42/none\endcsname{0.94}
\expandafter\def\csname R@sweepseed/192/s42/stop\endcsname{134}
\expandafter\def\csname R@sweepseed/192/s42/test\endcsname{0.57}
\expandafter\def\csname R@sweepseed/192/s7/inview\endcsname{0.22}
\expandafter\def\csname R@sweepseed/192/s7/none\endcsname{0.92}
\expandafter\def\csname R@sweepseed/192/s7/stop\endcsname{198}
\expandafter\def\csname R@sweepseed/192/s7/test\endcsname{0.56}
\expandafter\def\csname R@sweepseed/48/s0/inview\endcsname{2.00}
\expandafter\def\csname R@sweepseed/48/s0/none\endcsname{1.55}
\expandafter\def\csname R@sweepseed/48/s0/stop\endcsname{63}
\expandafter\def\csname R@sweepseed/48/s0/test\endcsname{1.61}
\expandafter\def\csname R@sweepseed/48/s42/inview\endcsname{1.94}
\expandafter\def\csname R@sweepseed/48/s42/none\endcsname{1.48}
\expandafter\def\csname R@sweepseed/48/s42/stop\endcsname{63}
\expandafter\def\csname R@sweepseed/48/s42/test\endcsname{1.54}
\expandafter\def\csname R@sweepseed/48/s7/inview\endcsname{1.86}
\expandafter\def\csname R@sweepseed/48/s7/none\endcsname{1.38}
\expandafter\def\csname R@sweepseed/48/s7/stop\endcsname{80}
\expandafter\def\csname R@sweepseed/48/s7/test\endcsname{1.43}
\expandafter\def\csname R@sweepseed/96/s0/inview\endcsname{0.55}
\expandafter\def\csname R@sweepseed/96/s0/none\endcsname{0.98}
\expandafter\def\csname R@sweepseed/96/s0/stop\endcsname{184}
\expandafter\def\csname R@sweepseed/96/s0/test\endcsname{0.90}
\expandafter\def\csname R@sweepseed/96/s42/inview\endcsname{1.31}
\expandafter\def\csname R@sweepseed/96/s42/none\endcsname{1.55}
\expandafter\def\csname R@sweepseed/96/s42/stop\endcsname{49}
\expandafter\def\csname R@sweepseed/96/s42/test\endcsname{1.52}
\expandafter\def\csname R@sweepseed/96/s7/inview\endcsname{1.27}
\expandafter\def\csname R@sweepseed/96/s7/none\endcsname{1.42}
\expandafter\def\csname R@sweepseed/96/s7/stop\endcsname{77}
\expandafter\def\csname R@sweepseed/96/s7/test\endcsname{1.40}
\makeatother

